Inferring Catchment in Internet Routing

BGP is the de-facto Internet routing protocol for exchanging prefix reachability information between Autonomous Systems (AS). It is a dynamic, distributed, path-vector protocol that enables rich expressions of network policies (typically treated as secrets). In this regime, where complexity is interwoven with information hiding, answering questions such as "what is the expected catchment of the anycast sites of a content provider on the AS-level, if new sites are deployed?", or "how will load-balancing behave if an ISP changes its routing policy for a prefix?", is a hard challenge. In this work, we present a formal model and methodology that takes into account policy-based routing and topological properties of the Internet graph, to predict the routing behavior of networks. We design algorithms that provide new capabilities for informative route inference (e.g., isolating the effect of randomness that is present in prior simulation-based approaches). We analyze the properties of these inference algorithms, and evaluate them using publicly available routing datasets and real-world experiments. The proposed framework can be useful in a number of applications: measurements, traffic engineering, network planning, Internet routing models, etc. As a use case, we study the problem of selecting a set of measurement vantage points to maximize route inference. Our methodology is general and can capture standard valley-free routing, as well as more complex topological and routing setups appearing in practice.

==> Conclusions.tex <==
In this work, we proposed and studied a methodology to infer routing behavior in the Internet for existing or hypothetical topological and routing configurations. Our methodology deviates from and enhances existing approaches, by predicting \ppoint catchment with certainty or probabilistically, with or without measurements, and under generic routing assumptions. Our approach is applicable in a number of practical use cases. Moreover, it can provide useful insights on BGP dynamics, which, if coupled with existing measurement approaches, can lead to the design of more efficient and lightweight techniques for measuring Internet routing.

\vkotronis{As future work, we plan to (i) investigate machine-learning approaches that learn the best action (e.g., prepending a path announcement, poisoning a route or activating a dormant anycast site) to affect catchment based on current measurement data and inference hints, 
%(ii) run measurement campaigns using the PEERING testbed~\cite{schlinker2014peering} for announcing paths on the control plane and RIPE Atlas for measuring them on the data plane, 
and (ii) derive approximation guarantees for the problem of efficient measurements  (see Section~\ref{sec:max-inf-catch-problem}).}

%In this work, we presented and studied, both analytically and experimentally, a model and methodology that enable the inference of routing behavior, emphasizing in catchment, in the policy-governed AS-level Internet. The employed approach is generic and can be extended to address a variety of topological and routing setups. The completeness/accuracy of inference can be significantly extended by taking into account VF violations as well as low-level BGP mechanisms besides policies (such as shortest path preference); targeted measurements may alternatively increase completeness by one order of magnitude in certain scenarios. Besides certain inference, we introduce a probabilistic approach as a promising technique to employ when using data with inherent sources of uncertainty, such as AS-level graph approximations~\cite{gill2012modeling}. We believe that this work can be coupled with other measurement-based estimation and inference approaches, assisting related research in the field.

==> Extensions.tex <==
%Here, we discuss how some Internet routing setups that might appear in practice, and are more complex than assumed in Section~\ref{sec:vf-model}, can be still captured by our model increasing the accuracy/completeness of inference. In Section~\ref{sec:disc-app} we further elaborate on potential applications of our methodology.

%To find real anycasters and anycasted prefixes, 
% We employ CAIDA's \texttt{pfx2as} dataset~\cite{caidapfx2as}, which maps IP prefixes to the ASes that advertise them in BGP, explicitly marking anycasted prefixes. We download BGP RIBs from RouteViews and RIPE RIS collectors via BGPStream, and focus on anycasted prefixes 
% %in the \texttt{pfx2as} dataset 
% for which: more than 40\% of the total RouteViews-RIPE RIS monitors (i.e., ASes) have seen at least one path towards the anycasters (\textit{visibility constraint}), and the measured catchment of any anycaster for a specific anycasted prefix is less than 90\% (\textit{plausible anycast constraint}). In total, we have information for 326 such prefixes.

% strict - same_color-acc - AVG 58.54394690071461
% strict - same_color-acc - MED 59.088122605363985


% strict - coverage - AVG 29.101390373226508
% strict - coverage - MED 22.36111111111111


% weak - same_color-acc - AVG 64.05665422747663
% weak - same_color-acc - MED 67.46987951807229


% weak - coverage - AVG 64.94483785299037
% weak - coverage - MED 68.70229007633588


\pavlos{ under work...}

%\vkotronis{Our work is applicable in multiple setups and use cases that might appear in the Internet. Being orthogonal to the model of inter-domain routing and underlying graph, it can encapsulate the following sub-cases:}

\subsection{\camera{Internet Routing Models}}\label{sec:disc-beyond}
\camera{We discuss how the model of Section~\ref{sec:model} can capture some common routing setups that are more complex than the VF model (Section~\ref{sec:vf-model}). Using our methodology on top of a more detailed model, can lead to higher accuracy/completeness of inference, as shown in Section~\ref{sec:real-evaluation}. We identify a future research direction (which could be facilitated by our framework) towards more accurate Internet models and routing inference.}

\myitem{\camera{Networks connected at multiple \ppoints.}} \camera{A network $i$ might connect to a network $j$ at more than one points (\eg at two IXPs), and have different preferences for those connections or even apply entirely different routing policies per point. \textit{Model modification:} Represent $j$ with more than one nodes in $\mathcal{G}$, and connect each of them to $i$ (at different \ppoints).} 

\myitem{\camera{Distributed/Large ASes.}} \camera{Large ASes might apply different policies at different parts in the world, due to distribution of routing equipment, PoPs, etc.~\cite{willinger2013internet}. Similarly, large ASes with complex internal structure may behave differently in different parts of their network~\cite{muhlbauer2006building}. 
\textit{Model modification:} Represent the distributed AS with multiple nodes (with different policies) \eg similar to the ``quasi-routers'' approach of~\cite{muhlbauer2006building}. In practice, only a small number of ASes (mainly Tier-1 ISPs) may need to be represented in such a way~\cite{muhlbauer2006building}.
}

\myitem{\camera{Per-prefix policies.}} \camera{Some networks apply different policies per prefix (of the same destination network $n_{dst}$)~\cite{anwar2015investigating%,willinger2013internet
}. \textit{Model modification:} Build a different \Rgraph per prefix.}

% The accuracy of the proposed methodology depends on how complete and accurate the knowledge of the routing policies $\mathcal{Q}$ and $\mathcal{H}$ is (perfect knowledge leads to $100\%$ inference accuracy). We verified this by comparing our inference results against real BGP RIBs collected from RIPE RIS~\cite{riperis} and RouteViews~\cite{routeviews} for %. Specifically, we considered 
% $\sim300$ %326
% prefixes that are anycasted in the Internet~\cite{caidapfx2as}. When using the VF model~\cite{gao2001stable} and the available AS-relationships~\cite{caidaasrel}, the achieved accuracy (for networks whose RIBs are available) is 60-70\%\footnote{An interesting observation is that introducing shortest path preference increases the inference completeness from  25\% to 70\%, while preserving the same accuracy.}, which complies with the observed accuracy of the VF-model for Internet routing~\cite{anwar2015investigating}. Introducing refinements (as those discussed above) in the routing policies for some nodes, increases accuracy; we tested this by considering per-prefix policies, similarly to~\cite{anwar2015investigating}. Inspired by these preliminary results, we plan to investigate how targeted measurements, \eg focusing on high-impact links close to the \Rgraph's root, can efficiently
% improve 
% %inference 
% accuracy.
%VK: I commented it out
%\pavlos{The accuracy of our methodology relates to the accuracy of the underlying model of routing policies: (i) For the subset nodes with certain inference, the accuracy is the same. However, with our methodology one can tell which nodes has certain inference, whereas with simulation-based methods (a) all nodes may appear to have a certain color (under a single simulation run), or (b) need many re-runs to find out which nodes have uncertain inference (and still not the complete set, neither the probabilities), or (c) considering only those with 1 eligible path (to infer certain inference nodes) results to an order of magnitude less nodes identified.} \vkotronis{Could you rephrase the purple text for clarity? Also check if you can shorten it, assuming we put it here.}


% \myitem{Comparison with ground truth in a semi-VF Internet.} We examine anycasted prefixes in CAIDA's prefix-to-AS (\texttt{pfx2as}) dataset~\cite{caidapfx2as} and consider as ground truth the associated entries of the BGP RIBs downloaded from RIPE RIS and RouteViews route collectors. We observe that using either the basic model alone, or in concert with Assumption~\ref{assumption:shortest-paths}, yields similar accuracy levels in the range of 60-70\%. The latter approach, which is more in-line with BGP operations, achieves a completeness of 70\% in contrast to 20-30\% of the former. These values comply with the accuracy and completeness estimates of assuming a VF-model for Internet routing~\cite{anwar2015investigating}. They can only be improved with more targeted/complex models and per-case adjustments as we describe in the following.

% \myitem{Integrating valley-free violations.} The model of Section~\ref{sec:vf-model} enables an evaluation of Internet setups, given only the AS-relationships. In practice, if the policies of a certain network $i$ do not conform to VF assumptions, the parameters $q_{i*}$ and $r_{i**}$ can be changed for this node. Extended policy models (beyond VF) could be applied by integrating approaches such as~\cite{kloti2015policy}. To deal with limited inference accuracy (see above) under VF assumptions, targeted measurements can be employed~\cite{anwar2015investigating}, \eg focusing on high-impact links close to the DAG's root.

% We validate (i) pure policy-based inference, and (ii) policy-based inference in combination with shortest path preference. 
% Approach (ii) is more in-line with classic BGP operation, offering more constrained path choices than (i), and thus more opportunities for certain inference. This is reflected in the accuracy and completeness levels; approach (i) yields values of $\sim$60\% and 29\% in terms of accuracy and completeness, respectively, while the respective values for (ii) are $\sim$67\% and 69\%.
% %Typically, both approaches yield --on average-- an accuracy of \red{$\sim$60-70\%}, 
% These values comply with the accuracy and completeness estimates of assuming a VF-model for Internet routing~\cite{anwar2015investigating}. 
% %However, ``pls'' has a completeness/coverage of \red{70\%} in contrast to ``pl'' with \red{30\%}; this is because ``pl'' offers more constrained path choices (best shortest paths), and thus more opportunities for certain inference. 
% We would like to stress that such results are the best we can reach with the \emph{given VF assumptions}, and can only be improved with more targeted/complex models; such models which are inconclusive and under investigation by the research community~\cite{giotsas2014inferring, anwar2015investigating}, can be fed into our approach.
% %which captures more generic setups than VF routing (see Section~\ref{sec:disc-beyond}).

% \subsection{Applications of Catchment Prediction}
% \label{sec:disc-app}

% Catchment prediction can be useful in a number of applications. In the following, we discuss some examples.

\subsection{\camera{Applications}}
\camera{Our inference framework could be applied to several network management processes; some examples are discussed below.}


\myitem{TE / Anycast design.} An operator can test hypothetical scenarios of how to announce a prefix, \eg from different combinations of \ppoints or doing AS-path prepending or poisoning \vkotronis{(\eg removing certain nodes and edges from the \Rgraph)}, and predict catchment with our methodology. Hence, load balancing or anycast strategies can be designed before actually changing the network configuration, \vkotronis{and can be further refined after deployment (when \eg additional measurement data become available).}
%of course, after deployment, they can be further refined. 
\vkotronis{Consider the following indicative example involving TE via path prepending. A $n_{dst}$ announces the same prefix $P$ differently to its two upstream providers / \ppoints $m1$ and $m2$, as $[n_{dst}]\rightarrow{P}$ and $[n_{dst}, n_{dst}, ..., n_{dst}]\rightarrow{P}$ respectively, aiming to increase the traffic through $m1$ since paths through $m2$ will be longer and de-preferred by some nodes. The longer the prepending, the less the catchment of $m2$. However, \textit{how many times does $n_{dst}$ need to prepend its ASN to achieve the desired balance between the catchment of its \ppoints}? Algorithm~\ref{alg:transform-vf-bn-weak} allows to answer the above question efficiently (with low computational complexity). First, note that path prepending can be captured in the \Rgraph by adding a number of ``virtual'' nodes (equal to the number of extra prepended ASNs) between $n_{dst}$ and $m2$. Apart from this change, the \Rgraph remains the same, since the eligible paths are independent of the path lengths. Hence, we can create a \Rgraph for each path prepending option, simply by duplicating the original \Rgraph and adding the corresponding number of virtual nodes. Then, for each \Rgraph we can apply Algorithms~\ref{alg:transform-vf-bn-weak} and~\ref{alg:coloring-vf-graph} to infer the catchment of the \ppoints. The complexity of this task is much lower than performing BGP simulations for each prepending case (which would be required by existing approaches). For instance, to examine $K$ path prepending scenarios would require $K$ BGP simulations of complexity $O(|\mathcal{N}|\cdot |\mathcal{E}|)$, whereas we need to run \textit{only once} Algorithm~\ref{alg:build-vf-graph} of complexity $O(|\mathcal{N}|\cdot |\mathcal{E}|)$ and then run $K-1$ times Algorithms~\ref{alg:transform-vf-bn-weak} and~\ref{alg:coloring-vf-graph} whose complexity is $O(|\mathcal{N}|+ |\mathcal{E}|)$ (which is $\ll O(|\mathcal{N}|\cdot |\mathcal{E}|)$ in all practical scenarios).
}


%\myitem{Traffic Engineering and Anycast Service Design.} Select how to announce a prefix (prepending, MED tuning~\cite{ciscobestpath}) to achieve the desired balancing of traffic load among the anycast sites.

\vkotronis{@pavlos: maybe we can get rid of the following since we already mention them in conclusions. For me it seems better to focus on a concrete app like TE anycast design with prepending, instead of branching out and disorienting the reader.}

\myitem{Peering policies.} Establishing a new connection with a peer network, can significantly change the catchment of \ppoints~\cite{lodhi2015complexities}. Predicting the impact of a new peering can provide insights for the most economically efficient peering decisions. 
%\myitem{Peering Policies.} Decide, based on the effect it will have to catchment and thus the incoming traffic, whether to start or end a peering connection and with which network (or IXP)~\cite{lodhi2015complexities}.

\myitem{Resilience.} Catchment prediction can be used to evaluate the resilience of a network against a failure of an \ppoint; \eg whether a link failure can overload border routers in other points. Similarly, the vulnerability of a network to BGP hijacking can be estimated, by mapping a hijacker to an ``illegitimate'' \ppoint.
%\vkotronis{, with expected impact equal to its catchment}. 

\myitem{DDoS mitigation.} DDoS protection organizations 
engage in IP anycast (and/or DNS redirection) to attract and scrub DDoS traffic destined to a victim network. These organizations can select where to deploy their ingress points to maximize their catchment, and thus best protect their customers.

% VK: commenting out, no space
%\vkotronis{@pavlos: check if you want to add 1-2 more apps from your suggestions in Section 9. For me these 4 are quite OK, we can add more "exotic" ones in future work.}

% announce the prefix of a victim network to attract (and scrub) the DDoS traffic. These organization can select where to deploy their ingress (or, ``attraction'') points, to best protect their customers, by selecting \ppoints that maximize their catchment.
% \myitem{Network Resilience.} Evaluate the resilience of the network to a failure of an \ppoint (\eg a peering link or border router), and how this would affect the traffic; for example, predict whether a failure in the link with an upstream would overload the links with other networks. 
% %This is complementary to investigating how many links should fail before communication is totally crippled~\cite{kloti2015policy}. 
% This could also be applied on evaluating BGP prefix hijacks, by inferring how much catchment a hijacker, i.e., an ``illegitimate'' \ppoint, could achieve w.r.t. to the victim which aims to achieve $\sim$100\% catchment. The inverse problem could be studied in the context of organizations offering DDoS protection; such organizations aim to achieve maximal catchment on their own \ppoints to attract DDoS traffic away from the victim.


%All the above modifications can be applied in combination.

%\pavlos{
%Similarly to the majority of related work, in our evaluation we used coarse estimates of the routing policies, based on the available AS-relationship data. This method offers an easy way to evaluate Internet routing, but its accuracy is limited. However, as we showed in ...our results in Section~\ref{}... by providing more accurate estimates of the policies for a subset of nodes, can significantly increase accuracy. Such estimates can be collected by targeted measurements and/or analysis of available data (\eg BGP messages, traceroute measurements). Although this is out of the scope of this initial study, we believe that it is an interesting research direction.
%}



==> Extensions_backup.tex <==
Here, we discuss how some Internet routing setups that might appear in practice, and are more complex than assumed in Section~\ref{sec:vf-model}, can be still captured by our model increasing the accuracy/completeness of inference. In Section~\ref{sec:disc-app} we further elaborate on potential applications of our methodology.
%In this section, we discuss issues related to the applicability of the proposed model and methodology in Internet routing setups that are more complex than assumed in Section~\ref{sec:model}.

% \subsection{Comparison to Ground Truth.}
% \label{sec:comp-with-gt}

%To find real anycasters and anycasted prefixes, 
% We employ CAIDA's \texttt{pfx2as} dataset~\cite{caidapfx2as}, which maps IP prefixes to the ASes that advertise them in BGP, explicitly marking anycasted prefixes. We download BGP RIBs from RouteViews and RIPE RIS collectors via BGPStream, and focus on anycasted prefixes 
% %in the \texttt{pfx2as} dataset 
% for which: more than 40\% of the total RouteViews-RIPE RIS monitors (i.e., ASes) have seen at least one path towards the anycasters (\textit{visibility constraint}), and the measured catchment of any anycaster for a specific anycasted prefix is less than 90\% (\textit{plausible anycast constraint}). In total, we have information for 326 such prefixes.

% strict - same_color-acc - AVG 58.54394690071461
% strict - same_color-acc - MED 59.088122605363985


% strict - coverage - AVG 29.101390373226508
% strict - coverage - MED 22.36111111111111


% weak - same_color-acc - AVG 64.05665422747663
% weak - same_color-acc - MED 67.46987951807229


% weak - coverage - AVG 64.94483785299037
% weak - coverage - MED 68.70229007633588

\subsection{Extensions of Basic Model in the Wild.}
\label{sec:disc-beyond}

% In this section, we discuss how some Internet routing setups that might appear in practice, and are more complex than assumed in Section~\ref{sec:model}, can be still captured by our model.
% %In this section, we discuss issues related to the applicability of the proposed model and methodology in Internet routing setups that are more complex than assumed in Section~\ref{sec:model}.

\myitem{Comparison with ground truth in a semi-VF Internet.} We examine anycasted prefixes in CAIDA's prefix-to-AS (\texttt{pfx2as}) dataset~\cite{caidapfx2as} and consider as ground truth the associated entries of the BGP RIBs downloaded from RIPE RIS and RouteViews route collectors. We observe that using either the basic model alone, or in concert with Assumption~\ref{assumption:shortest-paths}, yields similar accuracy levels in the range of 60-70\%. The latter approach, which is more in-line with BGP operations, achieves a completeness of 70\% in contrast to 20-30\% of the former. These values comply with the accuracy and completeness estimates of assuming a VF-model for Internet routing~\cite{anwar2015investigating}. They can only be improved with more targeted/complex models and per-case adjustments as we describe in the following.

\myitem{Integrating valley-free violations.} The model of Section~\ref{sec:vf-model} enables an evaluation of Internet setups, given only the AS-relationships. In practice, if the policies of a certain network $i$ do not conform to VF assumptions, the parameters $q_{i*}$ and $r_{i**}$ can be changed for this node. Extended policy models (beyond VF) could be applied by integrating approaches such as~\cite{kloti2015policy}. To deal with limited inference accuracy (see above) under VF assumptions, targeted measurements can be employed~\cite{anwar2015investigating}, e.g., focusing on high-impact links close to the DAG's root.

\myitem{Networks connected at multiple \ppoints.} A network $i$ might connect to a network $j$ at more than one points (\eg at two IXPs), and even apply different routing policies per point. \textit{Model modification:} Represent $j$ with more than one nodes in $\mathcal{G}$, and connect each of them to $i$ (at different \ppoints). 

\myitem{Distributed ASes.} Large ASes might apply different policies at different parts in the world, due to distribution of routing equipment, PoPs, etc.~\cite{willinger2013internet}. \textit{Model modification:} Represent the distributed AS with multiple nodes (with different policies). \red{In the special case of siblings, aggregate the nodes into one.}

\myitem{Per-prefix policies.} Some networks apply different policies per prefix (of the same destination network $n_{dst}$)~\cite{willinger2013internet}. \textit{Model modification:} Build a different \Rgraph per prefix.

% We validate (i) pure policy-based inference, and (ii) policy-based inference in combination with shortest path preference. 
% Approach (ii) is more in-line with classic BGP operation, offering more constrained path choices than (i), and thus more opportunities for certain inference. This is reflected in the accuracy and completeness levels; approach (i) yields values of $\sim$60\% and 29\% in terms of accuracy and completeness, respectively, while the respective values for (ii) are $\sim$67\% and 69\%.
% %Typically, both approaches yield --on average-- an accuracy of \red{$\sim$60-70\%}, 
% These values comply with the accuracy and completeness estimates of assuming a VF-model for Internet routing~\cite{anwar2015investigating}. 
% %However, ``pls'' has a completeness/coverage of \red{70\%} in contrast to ``pl'' with \red{30\%}; this is because ``pl'' offers more constrained path choices (best shortest paths), and thus more opportunities for certain inference. 
% We would like to stress that such results are the best we can reach with the \emph{given VF assumptions}, and can only be improved with more targeted/complex models; such models which are inconclusive and under investigation by the research community~\cite{giotsas2014inferring, anwar2015investigating}, can be fed into our approach.
% %which captures more generic setups than VF routing (see Section~\ref{sec:disc-beyond}).

\subsection{Applications}
\label{sec:disc-app}

\myitem{Traffic Engineering and Anycast Service Design.} Select how to announce a prefix (prepending, MED tuning~\cite{ciscobestpath}) to achieve the desired balancing of traffic load among the anycast sites.

\myitem{Peering Policies.} Decide, based on the effect it will have to catchment and thus the incoming traffic, whether to start or end a peering connection and with which network (or IXP)~\cite{lodhi2015complexities}.

\myitem{Network Resilience.} Evaluate the resilience of the network to a failure of an \ppoint (e.g., an inter-domain link or border router), and how this would affect the traffic; for example, predict whether a failure in the link with an upstream would overload the links with other networks. 
%This is complementary to investigating how many links should fail before communication is totally crippled~\cite{kloti2015policy}. 
This could also be applied on evaluating BGP prefix hijacks, by inferring how much catchment a hijacker, i.e., an ``illegitimate'' \ppoint, could achieve w.r.t. to the victim which aims to achieve $\sim$100\% catchment. The inverse problem could be studied in the context of organizations offering DDoS protection; such organizations aim to achieve maximal catchment on their own \ppoints to attract DDoS traffic away from the victim.


%All the above modifications can be applied in combination.

%\pavlos{
%Similarly to the majority of related work, in our evaluation we used coarse estimates of the routing policies, based on the available AS-relationship data. This method offers an easy way to evaluate Internet routing, but its accuracy is limited. However, as we showed in ...our results in Section~\ref{}... by providing more accurate estimates of the policies for a subset of nodes, can significantly increase accuracy. Such estimates can be collected by targeted measurements and/or analysis of available data (\eg BGP messages, traceroute measurements). Although this is out of the scope of this initial study, we believe that it is an interesting research direction.
%}


%%%%% OLD (DETAILED) TEXT BY VK %%%%%


% In this section, we describe how the proposed model and methodology could be extended to address several challenges beyond the scope of this paper, such as the fact that Autonomous Systems are not atomic nodes, and that inter-domain routing policies can be actually much richer --and more complex-- than the assumed VF policies. We thus discuss how our findings could be generalized in different Internet setups.

% \subsection{Networks with Multiple Peering Points.}

% \myitem{Setup.} Node $i$ having multiple peering points with node $j$, even with different relationships per point.

% \myitem{Solution.} Assuming that $i$ has $PP_{i,j}$ peering points with $j$, break $i$ into $|PP_{i,j}|$ virtual nodes $i_{k,j}$, $k=1,..,|PP_{i,j}|$, each of them having one peering point with $j$ (with the corresponding relationship), and the same peering points as $i$ with the rest of the nodes peering with $i$. Then form an additional node $i_{j}$, connected to all $i_{k,j}$ nodes via a default $c2p$ relationship as a traffic sink.

% \subsection{Distributed Networks.}

% \myitem{Setup.} Node/network $i$ having different connectivity at different points in the world, due to distribution of routing equipment, PoPs, etc.

% \myitem{Solution.} Similar to the previous setup, break node $i$ into multiple nodes according to the required distribution level (e.g., consistent policies in Asia different than Europe different than the US, etc.).

% \subsection{Per-prefix Policies.}

% \myitem{Setup.} Some --or all-- nodes engage in per-prefix specific --VF-- policies.

% \myitem{Solution.} Consider a different graph per prefix and apply the methodology on each prefix-specific graph.

% \subsection{Non-VF Policies.} 

% \myitem{Setup.} Some --or all-- nodes engage in different than VF policies.

% \myitem{Solution.} Modify/extend the policy-compliant NFA and re-apply it to transform the initial graph (or subgraphs if different policies apply per subgraph). Note that a limitation of the current transform is that the policy (or policies) should be expressible with a regular expression; however, a wide class of such policies, including popular VF extensions~\cite{cxp_paper} falls in this category.  

% \subsection{Per-prefix non-VF policies.}

% \myitem{Setup.} Some --or all-- nodes engage in different than VF policies on a per-prefix level.

% \myitem{Solution.} Combine the approaches of the last 2 setups, by considering prefix-specific graphs and NFA extensions together.

% \subsection{Combinations in the Wild.}

% As described in the last example, the previous setups can appear combined in the wild (e.g., distributed networks with several peering points with their peers, providers, or customers, conforming to a mixture of VF and non-VF per-prefix policies); correspondingly, the proposed solutions/extensions could be applied in combination to deal with these setups. 


%The proposed model and methodology are general enough to address the aforementioned cases.

==> Introduction_backup.tex <==

\subsection{Applications}
\myitem{Traffic engineering and Anycast design.} Select how to announce a prefix (\ie from which peering points, or manipulation of BGP announcement), to achieve the desired balancing of traffic/load among the anycasting points. For example, select to which peers a prefix will be announced, do path prepending to increase the length in some announcement, or poisoning to avoid the catchment \vkotronis{parenthesis: is the catchment a well-known term in literature/community?} of a (direct or indirect) neighbor.

\myitem{Peering policies.} Decide, based on the effect it will have to the incoming traffic, whether to start or end a peering connection and with which network (or IXP). \vkotronis{I would also add to determine the type of the connection, since p2p and c2p have different characteristics; e.g., would it be better to connect to a new transit or simply increase my peering matrix in the IXP?}

\myitem{Network robustness.} Evaluate the robustness of the network to, \eg a failure of an edge router (or, in general of a peering point), and how this would affect the traffic. For example, would a failure in the link with an upstream overload the links with the other upstreams? Moreover, evaluate the vulnerability to hijacks, by calculating what percentage of traffic can a hijacker (which can be considered as an ``illegitimate'' peering point) attract. \vkotronis{I really like the mapping between hijacks and illegitimate peering points, this shows that the definition is quite general. Although, I think we need to be more specific and state that we can do it primarily for type-0 hijacks, or do you think the use case can be extended? Finally, maybe the paper we did with Rowan at ETH some years ago on the policy-compliant path diversity also fits here; the difference is that there we calculate feasible policy-compliant paths between two specific ``peering points'' (actually ASes), while here we are more interested in how the traffic would be redistributed to the rest peering points upon a routing failure.}

\myitem{DDoS protection services.} Organizations offering DDoS protections services (\eg Cloudflare), proceed to MOAS announcements of the attacked prefix, attract the traffic destined to it, scrub it, and tunnel it back to the victim AS. In this case, there are two virtual peering points whose catchment needs to be evaluated: the victim and the DDoS organization. How efficient (\ie w.r.t.~the fraction of the traffic it attracts) will a company be in protecting a given customer (potential victim) AS?

\subsection{Motivational Examples}
\begin{itemize}[leftmargin=*]
\item A regional ISP covering a region with two major cities, $city_{A}$ and $city_{B}$, is connected to a tier-1 ISP $t_{A}$ through its infrastructure at $city_{A}$. To avoid overloading its infrastructure in $city_{A}$, the regional ISP decides to interconnect with another tier-1 ISP $t_{B}$ at $city_{B}$, aiming to split its traffic load among its infrastructure in the two cities. However, after connecting with $t_{B}$, it observes that $90\%$ of the incoming traffic enters its network at $city_{B}$ and $10\%$ at $city_{A}$, hence without achieving the expected load balancing.

\item A network with a single upstream, establishes a new connection to an IXP to offload some of its traffic through the cost-effective peering with the members of the IXP. However, it observes that it still receives the traffic for most of its peers through its upstream rather than the IXP. 

\item A network has two edge routers, $r_{A}$ and $r_{B}$, with which it connects to multiple upstreams (different at each router). To reduce the load in $r_{A}$, it starts doing path prepending in the BGP announcements from $r_{A}$, so that the paths are longer and preferred by less networks. However, no matter how long the announced paths from $r_{A}$ are, the change in the load share between $r_{A}$ and $r_{B}$ is negligible.

\item A content provider does anycast from three sites, in Europe, US, and Asia. It wants to start anycasting from one more site, and needs to select where to place it and connect it, in order to achieve the desired catchment. While the estimation of the catchment is possible after having deployed the new site and starting anycasting~\cite{}, it does not know how to predict the catchment without an actual deployment so that it selects the best location for the new site.

\item A network has selected its routing policies, and achieved to load the incoming traffic between two edge routes $r_{A}$ and $r_{B}$. However, at a time point, and without any change in the local routing policies, the network observes that the load on router $r_{A}$ is significantly higher than the load on $r_{B}$. 
\end{itemize}
\subsection{Problem definition}
A network is connected through its edge router(s) to one or more other networks/ASes. We call each of these ASes a \textit{peering point} of the network. 

\vkotronis{this definition assumes that each AS is a single node. Also it does not take into account that an AS may have multiple peering points with the same AS, since an AS is in reality a distributed entity. So I propose the following, more generalized, definition, which does not change the problem statement but shields us (I think) a bit better.}.

\vkotronis{A network is connected through its edge router(s) to one or more other networks/ASes. We call these connection points, where an AS is connected to another AS, \textit{peering points}. Note that an AS may have multiple peering points with the same neighbor.}

\begin{problem}
Given a network that advertises the same prefix through a set of $\mathcal{N}$ peering points, how much traffic (\ie \#networks) will each of these peering points attract?
\end{problem}

\vkotronis{@pavlos: traffic is not equivalent to networks. I would simply restate the problem statement as how many and which networks would route their traffic towards each of these peering points.}

There are network/traffic monitoring tools and methodologies that can calculate the fraction of the traffic \vkotronis{networks} that would be attracted by each peering point $\mathcal{N}$, when all the peering points are operational (\ie have announced the prefix and/or receive traffic). \todo{Find existing solutions and related work.}

\myitem{Goal 1: Prediction.} The primary goal of this paper is to provide an answer to the above question, when some  of (or, all) the peering points are not operational or do not exist yet, \eg for planning purposes.  

\myitem{Goal 2: Smart monitoring.} The second goal of this paper is to go beyond the state-of-the-art, and calculate the traffic attracted by operational peering points, in a lightweight and scalable way (\eg without pinging all IP addresses of anycasted destinations as in~\red{[ref]}). \pavlos{The second goal is not studied in the current version of the draft. The remaining material focuses on Goal 1.} 

\myitem{Key idea.} The key idea is to use the available information (BGP, traceroutes, etc.) under the current network state, in order to predict the routing paths after some network/routing changes, \vkotronis{e.g., when a new anycast site is employed by a network to announce a certain prefix, or a new AS originates the same prefix as another AS, either due to misconfiguration or malicious intent}.


\subsection{Applications}
\myitem{Traffic engineering and Anycast design.} Select how to announce a prefix (\ie from which peering points, or manipulation of BGP announcement), to achieve the desired balancing of traffic/load among the anycasting points. For example, select to which peers a prefix will be announced, do path prepending to increase the length in some announcement, or poisoning to avoid the catchment \vkotronis{parenthesis: is the catchment a well-known term in literature/community?} of a (direct or indirect) neighbor.

\myitem{Peering policies.} Decide, based on the effect it will have to the incoming traffic, whether to start or end a peering connection and with which network (or IXP). \vkotronis{I would also add to determine the type of the connection, since p2p and c2p have different characteristics; e.g., would it be better to connect to a new transit or simply increase my peering matrix in the IXP?}

\myitem{Network robustness.} Evaluate the robustness of the network to, \eg a failure of an edge router (or, in general of a peering point), and how this would affect the traffic. For example, would a failure in the link with an upstream overload the links with the other upstreams? Moreover, evaluate the vulnerability to hijacks, by calculating what percentage of traffic can a hijacker (which can be considered as an ``illegitimate'' peering point) attract. \vkotronis{I really like the mapping between hijacks and illegitimate peering points, this shows that the definition is quite general. Although, I think we need to be more specific and state that we can do it primarily for type-0 hijacks, or do you think the use case can be extended? Finally, maybe the paper we did with Rowan at ETH some years ago on the policy-compliant path diversity also fits here; the difference is that there we calculate feasible policy-compliant paths between two specific ``peering points'' (actually ASes), while here we are more interested in how the traffic would be redistributed to the rest peering points upon a routing failure.}

\myitem{DDoS protection services.} Organizations offering DDoS protections services (\eg Cloudflare), proceed to MOAS announcements of the attacked prefix, attract the traffic destined to it, scrub it, and tunnel it back to the victim AS. In this case, there are two virtual peering points whose catchment needs to be evaluated: the victim and the DDoS organization. How efficient (\ie w.r.t.~the fraction of the traffic it attracts) will a company be in protecting a given customer (potential victim) AS?

==> Measurements_old.tex <==

The first challenge in the above problem is to calculate $\mathcal{N}_{C}(S)$. The set of nodes with certain color after the measurement, depends on the measurement results, \ie the colors of the certain nodes. \pavlos{For example, if node A has only two incoming edges from nodes B and C, and the color of C is red, then $\mathcal{N}_{C}(B) = \{A\}$ if the measurement shows that B is red \vkotronis{(I would not say that $\mathcal{N}_{C}(B) = \{A\}$ but: $A \in \mathcal{N}_{C}(B)$)}, and $\mathcal{N}_{C}(B)=\emptyset$ otherwise \vkotronis{(I would not say that $\mathcal{N}_{C}(B) = \emptyset$ but: $A \not\in \mathcal{N}_{C}(B)$)}}. Hence, we cannot determine $\mathcal{N}_{C}(S)$ unless we know the colors (\eg. by measurements or an oracle) for all nodes of $S$; we can calculate the set $\mathcal{N}_{C}(S)$, only conditional on the color of the nodes of $S$ (\eg using Algorithm~\ref{alg:coloring-from-measurements}), \ie $\mathcal{N}_{C}(S| i\rhd ,~\forall i\in S)$. \pavlos{An approach is to take the average over all the possible color combinations of nodes in $S$; this would require to evaluate/calculation $\mathcal{N}_{C}(S)$ a number of $|PP|^{|S|}$ times, which is exponential on the set size of $S$. Moreover, calculating the exact probabilities $P\{i \rhd \}$ is NP-hard itself (see Section~\ref{} -- discussion to be added).}

\myitem{Sequential vs. Concurrent measurements.} The above discussion reveals that Problem~\ref{problem:budgeted-measurements} can further differentiate if considered under \textit{sequential} or \textit{concurrent} measurements (in the former case, the result of the first measurement can provide further information about how to perform the second measurement, etc.) \pavlos{Some examples (in figures) could help here to demonstrate why these cases differentiate; but it's not a crucial task, leave it for later.} 

\myitem{Full-path vs. Single-node measurements.} Another differentiation comes of the fact that measurements can be \textit{full path} (\ie traceroute or BGP path) or \textit{single node} (\ie ping) measurements. However, in this case, the only difference is that in the former case, measuring a set of nodes $S$ gives us information about the paths of all intermediate nodes in the measured path. If we define as $\bar{S} = \{k:k\in path_{ij}, \forall i\in S\}$, the set $\mathcal{N}_{C}(S)$ with full path measurements is equal to the set $\mathcal{N}_{C}(\bar{S})$ with single node measurements. \textit{Remark:} Note here that while $S\cap \mathcal{N}_{C}(\emptyset)=\emptyset$, the set $\bar{S}$ will always contain nodes with certain colors (\eg the peering points themselves), \ie $\bar{S}\cap \mathcal{N}_{C}(\emptyset)\neq \emptyset$. \vkotronis{I get the last observation but since it might be a bit confusing we can leave it out in the production text (not very important).}


\myitem{Calculating the node utility.} Let a set of measured nodes $S_{M}$ and the respective set of nodes with certain color $\mathcal{N}_{C}(S_{M})$.  We define the \textit{exact coloring utility} $U(i|S_{M})$ of a node $i\in$ as the extra number of nodes that can be colored with certain color, if a measurement from this node takes place, \ie 
\begin{equation}
U(i|S_{M}) = |\mathcal{N}_{C}(S_{M}\cup \{i\}) - \mathcal{N}_{C}(S_{M})|
\end{equation}
As discussed above, we might not be able to calculate the quantity 
$\mathcal{N}_{C}(S_{M}\cup \{i\}) $ unless we know the color of node $i$ (given that we know the colors of all nodes in $\mathcal{N}_{C}(S_{M})$). Hence we can only calculate for a $x\in PP_{j}$ the quantity
\begin{equation}
U(i|S_{M},i\rhd x) = |\mathcal{N}_{C}(S_{M}\cup \{i\}|i\rhd x) - \mathcal{N}_{C}(S_{M})|
\end{equation}
From the above expression, we can define the \textit{average} \vkotronis{maybe instead of $\pi_{i}(x)$ you mean $p_{i}(x)$ in the first expression as the probability of this node being of color $x$?}, \textit{min}, and \textit{max} utilities of a node $i$
\begin{align}
\bar{U}(i|S_{M}) &= \sum_{x\in PP_{j}}U(i|S_{M},i\rhd x) \cdot \pi_{i}(x)\\
U_{min}(i|S_{M}) &= \min_{x\in PP_{j}}U(i|S_{M},i\rhd x)\\
U_{max}(i|S_{M}) &= \max_{x\in PP_{j}}U(i|S_{M},i\rhd x)
\end{align}
The latter two quantities can be easily calculated from the existing information in the graph and using Algorithm~\ref{alg:coloring-from-measurements}. The former quantity needs the knowledge of the probabilities $\pi_{i}(x)$; given this information, it can be calculated in the same (easy) way as well. However, to calculate (and update, \eg after a measurement) these probabilities in the generic case, is a challenging task (NP-hard see Section~\ref{}). \pavlos{We can handle this with an approximation method for re-calculation of the probabilities $\pi_{i}(x)$. I will have some details in an earlier section.}

\myitem{Calculating the utility of a set of nodes.} If instead of a single node, we have a set of nodes $S_{M'}$ (let, w.l.o.g. $S_{M'}\cap S_{M}=\emptyset$), then the \textit{exact utility} is defined as
\begin{equation}
U(S_{M'}|S_{M}) = |\mathcal{N}_{C}(S_{M}\cup S_{M'}) - \mathcal{N}_{C}(S_{M})|
\end{equation}
and can be calculated only conditional to the coloring of all nodes in $S_{M'}$, \ie \begin{equation}
U(S_{M'}|S_{M},S_{M'}\rhd \mathbf{x})
\end{equation}
where $\mathbf{x}$ a vector of size $|S_{M'}|$ whose elements correspond to the colors of nodes $i$, $\forall i\in S_{M'}$.
The corresponding average/min/max utilities are
\begin{align}
\bar{U}(S_{M'}|S_{M}) &= \sum_{\mathbf{x}\in \{PP_{j}\}^{|S_{M'}|}}U(i|S_{M}, S_{M'}\rhd \mathbf{x}) \cdot \pi_{S_{M'}}(\mathbf{x})\\
U_{min}(S_{M'}|S_{M}) &= \min_{\mathbf{x}\in \{PP_{j}\}^{|S_{M'}|}}U(i|S_{M}, S_{M'}\rhd \mathbf{x})\\
U_{max}(S_{M'}|S_{M}) &= \max_{\mathbf{x}\in \{PP_{j}\}^{|S_{M'}|}}U(i|S_{M}, S_{M'}\rhd \mathbf{x})
\end{align}
To calculate the above utilities, we need to calculate the quantity $U(S_{M'}|S_{M},S_{M'}\rhd \mathbf{x})$ over all the possible values that $\mathbf{x}$ takes, \ie $|PP_{j}|^{|S_{M'}|}$ different cases, which is exponential to the size of the set $S_{M'}$ and becomes inefficient for large sets $S_{M'}$ (and/or for many peering points).

\myitem{Designing a greedy algorithm.} Summarizing the above discussion, the challenges for Problem~\ref{problem:budgeted-measurements} are: (i) there is no exact or approximation algorithm \pavlos{just a claim for the moment} given an oracle for the sets $\mathcal{N}_{C}(S)$, $S\subseteq\mathcal{N}_{BN}\backslash\mathcal{N}_{C}(\emptyset)$; (ii) the quantity $\mathcal{N}_{C}(S)$ cannot be calculated before doing the corresponding measurements (\ie an oracle does not exist), and (iii) even approximating the quantity $\mathcal{N}_{C}(S)$ with its statistics (average/min/max utility), leads to a calculation over a probability space that exponential to the size of $S$ and requires the exact probabilities $\pi_{i}(x)$, whose calculation is NP-hard in the general case. \pavlos{These clearly show that it is a fucking difficult problem :P}

We propose an algorithm for Problem~\ref{problem:budgeted-measurements}. Our design choices are driven by the aforementioned challenges. \pavlos{TODO: write explicitly the connection of each step/choice with one or more challenges.}
\begin{enumerate}
\item We proceed greedily, by selecting at each iteration a node to be measured.
\item We select the node with the highest average or min or max utility.
\item If possible to perform the measurement before proceeding further (\textit{sequential measurements}), we do the measurement. Otherwise (\textit{concurrent measurements}), \pavlos{we randomly assign a color to the current node $i$ according to the probabilities $\pi_{i}(x)$.} Then, we update the nodes with certain color (and the probabilities $\pi$ for the remaining nodes \pavlos{probably we will do this approximately}) 
\end{enumerate}



\myitem{Other heuristic algorithms.} \pavlos{Some ideas about heuristic algorithms are the following. TODO: formalize and elaborate and compare performance with sims.} 
\begin{itemize}
\item \textbf{Only path-length (\ie not coloring) based.} Instead of the utilities, we use only the (expected) number of nodes to be contained in the full-path measurement; \ie based on size of $\bar{S}\backslash\mathcal{N}_{C}(\emptyset)$ (but we don't know the exact $\bar{S}$ before the measurement). However, for all singletons $S$ we can calculate the minimum $\bar{S}\backslash\mathcal{N}_{C}(\emptyset)$ (over all possible paths) and start selecting greedily.
\item \textbf{Children cone size.} The most naive approach. However, this is also the least computational heavy. No measurements or calculations of coloring (or probabilities) is required.
\end{itemize}


==> Methodology.tex <==
Taking as approximation Eq.~\eqref{conjecture:anycast-path-in-best-paths}, we try to infer which of the paths $\{[path_{ij}, X]: j\in\mathcal{N}\}$ will be selected as $path_{iX}$.

\subsection{Rule 1: one common intermediate network.} 
Let two networks $i,k\in\mathcal{AS}\backslash \mathcal{N}$. If the network $k$ is in every path between $i$ and $j\in\mathcal{N}$, then $i$ will select the same peering point $j$ that the network $k$ selects. More formally, if
\begin{equation*}
k\in path_{ij},~~~\forall j\in\mathcal{N}
\end{equation*}
then
\begin{equation*}
path_{iX} = [path_{ik}, path_{kX}]
\end{equation*}

\textit{Remark:} The sub-path $path_{ik}$, will be the same in any path $path_{ij}$ (before and after the routing changes). \pavlos{this holds, right?}
\vkotronis{No it does not. E.g., imagine a routing change where $i$ selects another upstream to reach the prefix. Even if $k$ remains on the path, $path_{ik}$ might be different. However what does actually hold, is that $k$ dictates the right sub-path (so $k$ is the node that determines how the right sub-path looks like, at least at the first hop).}

\todo{Check if this holds in (i) sims and (ii) real data. If more than one ASes are common in all paths, e.g., k1 and k2, choose the one that is closer to $\mathcal{N}$. Maybe to check for all, we need to check recursively.}

\todo{Check how frequently such a case happens.}\pavlos{I suspect it (i) is rare and (ii) decreases with $N$}

Rule~1 is a strong rule that infers with certainty the paths for an AS $i$, given the knowledge for the paths of $k$.



\subsection{Rule 2: routing policy.}
Under the GR-model a network prefers to route traffic through a customer, then through a peer, and then through a provider. Let a network $i$ that receives routing paths to network $j$ through a customer network $C_{i}$, a peer network $P_{i}$, and a provider (upstream) network $U_{i}$. 

\myitem{Strict ordering.} Then, we define a \textit{strict inequality} of the paths as follows.
\begin{equation}
[i, C_{i}, ..., j] > [i, P_{i}, ..., j] > [i, U_{i}, ..., j]
\end{equation}
If $C1_{i}$ and $C2_{i}$ two customer networks of $i$ (similarly for peer and provider networks), and both advertise a path to $j$. Then these paths are \textit{equivalent}, and we denote
\begin{equation}
[i, C1_{i}, ..., j] \sim [i, C2_{i}, ..., j]
\end{equation}

\myitem{Weak ordering.} In the latter case, $i$ will prefer one of the two paths due to (i) local preferences or (ii) shorter path length. In this case we denote the \textit{weak inequality} of the two paths as
\begin{equation}
[i, C1_{i}, ..., j] \geq [i, C2_{i}, ..., j]
\end{equation}

\vspace{2\baselineskip} 
The available information about AS-relationships that is provided by the CAIDA dataset, allows us to proceed to a \textit{strict ordering} of paths. The \textit{weak ordering} requires further information that typically is not available. Hence, using only strict ordering, leads to more accurate results (but there are more equivalent paths, for which we cannot do an inference). \vkotronis{Correct. So we trade accuracy for coverage, right?}

\begin{conjecture}\label{conjecture:anycasting-path-not-worse-than-best-path}
The path from a network $i$ to $X$ (for $pfx_{X}$) is not ``smaller'' than any path from $i$ to a peering point $j$ of $X$  (for $pfx_{j}$) 
\begin{equation}
path_{iX} \geq path_{ij}, ~~\forall j\in\mathcal{N}
\end{equation}
\end{conjecture}

We verified that Conjecture~\ref{conjecture:anycasting-path-not-worse-than-best-path} always holds in our simulation results (see, \eg Fig.~\ref{fig:comparison-paths-next-hop-type-anycast}).

\todo{Mathematically prove Conjecture~\ref{conjecture:anycasting-path-not-worse-than-best-path} (under GR model).}

\todo{Check if Conjecture~\ref{conjecture:anycasting-path-not-worse-than-best-path} holds also in real data. For example
\begin{itemize}
\item Consider an AS $X$ and a prefix $pfx_{X}$, and all its neighbors $\mathcal{N}$ (select only those to which $X$ advertises $pfx_{X}$). Check paths of all available vantage points $i\in\mathcal{AS}$ to the prefixes $pfx_{X}$ and $pfx_{j}$, $j\in\mathcal{N}$.
\item AND/OR, consider a MOAS pfx and let the MOAS ASes be the set $\mathcal{N}$. Compare paths of all available vantage points $i\in\mathcal{AS}$ to the MOAS prefix and to the prefixes $pfx_{j}$, $j\in\mathcal{N}$.
\end{itemize}.
If violated, then why? (e.g., inaccurate AS-relationships data)
}


\subsection{Building the DAG}
Given the above analysis and discussion, one approach to infer routing paths is to find all paths a network $i$ sees and then infer the path that will be selected based on Rule 2 (or Rule 1). 

Hence, at first we need to find all the paths $path_{ij}$, $\forall \{(i,j):i\in\mathcal{AS}, j\in\mathcal{N}\}$. We can calculate these paths based on the GR model, or find them from real routing data that are available:

\myitem{DAG: GR model \& NFA graphs.} One way would be to simulate the AS topology with the GR model. However, this would require to know the local preferences (which we do not know) or to set them arbitrarily (which would lead to very inaccurate results\pavlos{how inaccurate? we could quantify?} \vkotronis{The only way I can think of is statistical testing with varying loc prefs, but since there is no accepted ground truth we can only try to validate through CAIDA's AS-level graph and BGPStream updates somehow.}). Therefore, we proceed with the following GR-based methodology:
\begin{enumerate}
\item We build the NFA graph. \pavlos{We will need to have some section earlier or here about the NFA. Leave this task for later, after we see if we use the NFA graph approach finally.} \vkotronis{Yes I agree. Actually we transform the AS-level graph using a policy NFA. I can add a section on how a graph is transformed so that we can run classic path algorithms and extract policy-compliant paths, referencing also the INFOCOM paper.}
\item We calculate all the valley free (VF) paths from the peering points to all ASes. \pavlos{Remark: In fact, we do not calculate all the VF paths, because this is a resource-heavy task (computation and memory) and leads to a graph with cycles. Hence, we calculate only all the \textit{preferred} VF paths. We need a section to describe what we do (selective DFS) and elaborate on the why. Leave this task for later as well.} \vkotronis{OK. The most important task actually is to formalize some of the statements we make earlier and back them up with both mathematical proof and sim data.}
\item We build a directed graph (DAG), with vertices the ASes, and root nodes the peering points. We add edges for each node $i$ as follows:
	\begin{itemize}
	\item From the set of all the first hop neighbors from the paths $path_{ij}$, $j\in\mathcal{N}$, find the subset $P(i)$ of first hop neighbors that are not $<$ than any other first hop neighbor.
	\item Add a directed edge $k\rightarrow i$, $\forall k\in P(i)$.
	\end{itemize}
\end{enumerate}

\myitem{DAG: real data \& AS relationships.} A second way to build a DAG, is directly by using routing information from BGP data and traceroute measurements. 
\begin{enumerate}
\item From each available vantage point $i\in\mathcal{VP}\subseteq\mathcal{AS}$ and peering point $j\in\mathcal{N}$, collect the paths $path_{ij}$, \ie in total $O\left(|\mathcal{VP}|\cdot |\mathcal{N}|\right)$. Let $\mathcal{PATHS}$ be the set of all these paths.
\item Build a directed graph with nodes the networks $i\in \{j\in path: path\in \mathcal{PATHS}\}$, and edges as follows: for each tuple in a path $[..., i, j, ...]$, add a directed edge $j\rightarrow i$
\item \todo{Check if this graph is acyclic (from data or prove with counterexample).} \pavlos{Probably not; or, at least it is not in the generic case. To remove cycles, proceed to the following step.}
\item Use the CAIDA dataset to find AS-relationships between nodes in the graph. For each node $i$ in the graph that has more than one incoming edges, find the set of predecessors $P(i)$ that are not $<$ than any other predecessor. Remove the edges $j\rightarrow i$, $\forall j \notin P(i)$.
\end{enumerate}

\todo{What is the coverage of this approach? How many ASes are in the DAG?}

\todo{Calculate the accuracy of this approach. I.e., for nodes with certain color, for how many of them the anycasting path is in the graph}

\pavlos{To include also nodes that do not exist in the $\mathcal{PATHS}$, we can augment this graph with the GR-DAG, and have a hybrid approach. Think about how to design such an approach.}

\pavlos{An idea is, instead of using the CAIDA dataset to try to infer the preference of a node to its predecessors from other real data. E.g., if a node consistently prefers paths for one of its predecessors (when all of them or some of them advertise the same prefix to it), then assign to this node a high preference. E.g., is a node seems to have equal preference and select by length size, then add higher preference to the predecessor that leads to a shorter path.}


\subsection{DAG-based inference}
\pavlos{Ideas about what to do with the DAG we have built (not all of them to be studied in a single paper):
\begin{itemize}
\item Color nodes and find uncolored nodes. Check coverage.
\item Do probabilistic coloring for uncolored nodes.
\item Do measurements or other analysis to decide for uncolored nodes.
\item Use base datasets, and apply some ML to decide for uncolored nodes, or assign edge weights (i.e., preferences)
\item Find the required measurement (i.e., all nodes whose policy needs to be identified to lead in a fully colored graph). Different flavors of measurements: (i) exhaustive (full coverage of the graph) or partial coverage, (ii) optimal set selection  or heuristic/approximation. Design an algorithm and test its performance with sims and/or real data.
\item Find important nodes (first define ``important'' and metrics of importance)
\end{itemize}
}






==> Model_backup.tex <==
\begin{itemize}
\item Network graph $\mathcal{G}(\mathcal{N},\mathcal{E},\mathcal{R}, \mathcal{Q})$
\item Node relationships $\mathcal{R} = \{r_{ij}: i,j\in\mathcal{N},e_{ij}\in\mathcal{E}\}$, a relationship can be \{\textit{c2p,p2p,p2c}\}. Note that if $r_{ij}=c2p$, then $r_{ji}=p2c$ (\textit{p2p} relationships are symmetric). They are assumed to be known.
\item Local preferences $\mathcal{Q} = \{q_{ij}: i,j\in\mathcal{N},e_{ij}\in\mathcal{E}\}$; a local preference can be captured by a number (as in Cisco routers),  or a semantic expression. Note that local preferences can be asymmetric. For the moment we assume that the local preferences are not known for our network.
\item AS-path from $i$ to $j$ $\aspath{i}{j}$; we also use the following notation \eg $\aspath{i}{j}=[i,x,y,...,j] = [i,x,\aspath{y}{j}]$
\item Network VF-BN graph $\mathcal{G}_{BN}(\mathcal{N}_{BN},\mathcal{E}_{BN}, \mathcal{Q})$
\item $\mathcal{M}$ peering points of the destination node
\item coloring/routing function $f:\mathcal{N}\rightarrow \mathcal{M}\cup \{0\}$, \eg $f(i)=m$ if we know that node $i\in\mathcal{N}$ routes traffic to the destination through the peering point $m\in\mathcal{M}$, and $f(i)=0$ if we are not sure about through which peering point the node $i$ routes its traffic.
\item $\pi_{i}(m)$ probability a node $i$ to route its traffic through the peering point $m$. In case $f(i)=m$, then $\pi_{i}(m)=1$ and $\pi_{i}(n)=0$ $\forall n\neq m$.
\end{itemize}


\myitem{Basics.} We assume a network with a set of nodes $\mathcal{N}$ and edges $\mathcal{E}$%
%
\footnote{In the remainder, unless otherwise stated, we consider that a node represents an AS, and an edge corresponds to a peering link between two ASes. However, this model could capture more complex setups appearing in the Internet, \eg distributed ASes could be represented by more than one nodes, or sibling ASes with a single node.}%
%
. Nodes use the BGP~\cite{bgprfc} (which is a \vkotronis{policy-based}, destination-oriented, path-vector protocol) to establish routing paths. Let a node $i$ advertise a prefix $pfx_{i}$. Let us denote as $path_{ji}$ the path selected by node $j$ to route traffic to node $i$ \vkotronis{Maybe it would be better to denote it in way so that $pfx_{i}$ is the actual destination rather than the node? This may help later with MOAS. Not totally sure though.}, \eg
\begin{equation*}
path_{ji} = [j,x,y,...,z,i],~~~i,j,x,y,..,z\in\mathcal{N}
\end{equation*}
and let us call the $path_{ji}$ as the ``best path'' from $j$ to $i$.

\myitem{Node relationships.} We consider the classic Gao-Rexford / valley-free model (VF-model) governing routing between nodes.
\vkotronis{Although this assumption may not always hold in the Internet (here cite philippa's and Giotsas's papers), it still applies to the vast majority of the AS-level relationships.}
Specifically, we assume each pair of nodes has either a \textit{customer-to-provider} or a \textit{peer-to-peer} relationship. Let us denote the sets of customers, peers, and providers (or, upstreams) of a node $i$, as $\mathcal{C}_{i}$, $\mathcal{P}_{i}$, and $\mathcal{U}_{i}$, respectively. We define the peering points of a node $i$, as the set of nodes $\mathcal{C}_{i}\cup\mathcal{P}_{i}\cup\mathcal{U}_{i}\equiv \{j\in\mathcal{N}: (i,j)\in\mathcal{E}\}$. \vkotronis{However, this definition does not capture setups where the same AS has a different relationship at different e.g., geo points around the world with another AS.}

Based on the inter-node relationships, each (directed) edge $e_{ij}\in\mathcal{E}$ can be classified as a
\begin{itemize}
\item \textit{c2p}, customer ($i$) to provider ($j$); or
\item \textit{p2p}, peer ($i$) to peer ($j$); or 
\item \textit{p2c}, provider ($i$) to customer ($j$).
\end{itemize}

\myitem{Routing policy.} Under the VF-model, when a node $i$ has a best path for node $j$ \vkotronis{best paths are for a prefix, since BGP is destination-based (not per node, but per prefix)} through a customer, it advertises this path to all its neighbors; and when the best path is through a peer or provider, node $i$ advertises this path only to its customers.

Moreover, a node prefers paths through a customer, more than paths through a peer; and paths through a peer more than paths through a provider. If paths are learned from more than one customers (or peers/providers), then the shortest path is preferred; and if these paths are of equal length, then the path with the highest local neighbor preference is preferred. \vkotronis{I think the last statement is wrong. Preference always comes first, then we have the length and afterwards miscellaneous tie-breakers (see best-path selection algorithm).}

To formalize these preferences, we define an ordering of path preference as follows. 

\myitem{Strict path ordering.} Let a node $i$ receive paths for node $j$ through a customer $c\in\mathcal{C}_{i}$, a peer $p\in\mathcal{P}_{i}$ , and a provider (upstream) $u\in\mathcal{U}_{i}$. We denote the preference of node $i$ to these paths, by defining path inequality:
\begin{equation}
[i, c, ..., j] \succ [i, p, ..., j] \succ [i, u, ..., j]
\end{equation}

If $i$ receives paths from two of its customers $c1,c2\in\mathcal{C}_{i}$ (similarly for peers or providers), we write that these paths are equivalent (or, of equivalent type), and denote
\begin{equation}
[i, c1, ..., j] \simeq [i, c2, ..., j] 
\end{equation}

\myitem{Weak path ordering.} In the latter case, $i$ will still prefer one of the two paths (\eg due to local neighbor preferences or shorter path lengths), let the path through $c1$. In this case we capture the preference between two paths of equivalent type, by denoting the weak path inequality as 
\begin{equation}
[i, c1, ..., j] \succeq [i, c2, ..., j] 
\end{equation}

==> Model_backup1.tex <==
\begin{table}
\centering
\caption{Important Notation.}\label{table:notation}
\begin{tabular}{l|l}
\hline
{$\mathcal{G}$} & {Network graph; $\mathcal{G}(\mathcal{N},\mathcal{E},\mathcal{R}, \mathcal{Q})$}\\
\hline
{$\mathcal{N}$} & {Set of nodes in $\mathcal{G}$}\\
\hline
{$\mathcal{E}$} & {Set of edges \vkotronis{$\mathcal{E} = \{e_{ij}, i,j \in \mathcal{N}\}$} in $\mathcal{G}$}\\
\hline
{$\mathcal{R}$} & {Node relationships $\mathcal{R} = \{r_{ij}: i,j\in\mathcal{N},e_{ij}\in\mathcal{E}\}$, }\\
{}&{$r_{ij}\in\{c2p,p2p,p2c\}$}\\
\hline
{$\mathcal{Q}$} & {Local preferences $\mathcal{Q} = \{q_{ij}\in\mathbb{R}: i,j\in\mathcal{N},e_{ij}\in\mathcal{E}\}$}\\
\hline
{$\aspath{i}{j}$}&{Path from node $i$ to node $j$}\\
\hline
{$\bestaspath{i}{j}$}&{Best path from node $i$ to node $j$}\\
\hline
{$\mathcal{M}$} & {Peering points of the destination node $n_{dst}$.}\\
\hline
{$i\rhd m$} & {Node $i$ is connected to $n_{dst}$ through the peering point $m$ %\vkotronis{Ambiguity here: I think you mean the peering point which shows as the last hop on paths from $i$ to $n_{dst}$ correct? Not the peering point with which $i$ is connected to the rest of the path? I know what you mean, but the reviewer may not :).}
}\\
\hline
{$f$} & {Routing function, \eq{eq:routing-function}}\\
\hline
{$\mathcal{G}_{BN}$} & {VF graph; $\mathcal{G}_{BN}(\mathcal{N}_{BN},\mathcal{E}_{BN})$}\\
\hline
{$\pi_{i}(m)$} & {Route probability for node $i$ and peering point $m$, \eq{eq:route-probability}.}\\
\hline
{$p_{ij}$} & {$Prob\{q_{ij}=\max_{k\in P_{i}}q_{ik}\}$, where $P_{i}$ the neighbors of $i$.}\\
\hline
\end{tabular}
\end{table}



\subsection{Network and Routing}
We assume a network with a set of nodes $\mathcal{N}$ and edges $\mathcal{E}$. A node represents an AS, and an edge corresponds to a link between two ASes%
%
\footnote{
%In the remainder, unless otherwise stated, we consider that a node represents an AS, and an edge corresponds to a peering link between two ASes. 
We model ASes as single nodes for presentation simplicity. However, the model can capture more complex setups appearing in the Internet: distributed ASes could be represented by more than one nodes, sibling ASes could be integrated in a single node, etc. \pavlos{we discuss these issues in section XX}}%
%
. We refer to the nodes connected with an edge to a node $i$, as the neighbors of $i$.

%\vkotronis{Maybe we need to state that we assume a simple BGP model, or that we assume proper BGP but focus only on the relevant aspects employed for policy-based routing from node $i$ to node $j$?}
%\footnote{In practice, nodes learn paths for a destination prefix, rather than a destination AS. Here, for simplicity and without loss of generality, we assume that the destination node announces only one prefix, and none of the other nodes in the network originate this prefix. \vkotronis{but the latter assumption counter the rest of the paper, did you have sth else in mind?}}
\myitem{Routing protocol.} Nodes use BGP~\cite{bgprfc} %(which is a \vkotronis{policy-based} path-vector protocol) 
to establish routing paths towards different Internet destinations. The main operation of BGP that is relevant to our study, is as follows. A destination node $n_{dst}$ announces a prefix. Every other node
%For a given destination node $n_{dst}$, a node 
$i$ learns from its neighbors paths to $n_{dst}$ (\ie its prefix), stores them in a local routing table (Routing Information Base, RIB), and selects one of them as its best path to $n_{dst}$ (according to, \eg its \textit{local preferences}). Then, $i$ may advertise this best path to its neighbors (according to its \textit{export policies}). 

A path contains a sequence of nodes; we denote a path from $i$ to $j$ as $\aspath{i}{j}$, and also use the following notation 
\begin{equation*}
\aspath{i}{j}=[i,x,y,...,z,j] %= [i,x,\aspath{y}{j}]
,~~~i,x,y,...,z,j\in\mathcal{N}
\end{equation*}
%\vkotronis{in order to represent paths in compact form. In this example, we learn that for this path $i$ employs $x$ to reach $j$.}
We further denote the best path from $i$ to $j$ (\ie the path in the RIB of $i$ that $i$ prefers to reach $j$) as $\bestaspath{i}{j}$.

\myitem{Node relationships.} Each pair of neighboring nodes has either a \textit{customer-to-provider} or a \textit{peer-to-peer} relationship%
%
\footnote{These are the main (business) relationship types between ASes in the Internet~\cite{gao-rexford}; while different relationships have been observed, they count for a very small fraction of the AS pairs~\cite{philippa}. \pavlos{We discuss how these other relationships/policies can be captured in our model in Section XX}.}%
%
. We denote the set of node relationships as $\mathcal{R} = \{r_{ij}: i,j\in\mathcal{N},e_{ij}\in\mathcal{E}\}$, with $r_{ij}\in \{\textit{c2p,p2p,p2c}\}$, where
\begin{itemize}
\item $r_{ij}=\textit{c2p}$, customer ($i$) to provider ($j$); or
\item $r_{ij}=\textit{p2p}$, peer ($i$) to peer ($j$); or 
\item $r_{ij}=\textit{p2c}$, provider ($i$) to customer ($j$).
\end{itemize}
Note that when $r_{ij}=c2p$ then $r_{ji}=p2c$, but \textit{p2p} relationships are symmetric.

In the remainder, we assume that the node relationships are known, and use the experimentally collected (and commonly used in related literature) CAIDA AS-relationship dataset~\cite{}.
 
\myitem{Routing policies.} A node, based on its routing policies, selects (a) a \textit{best path} to $n_{dst}$ out of the paths in its RIB (\ie learned from its neighbors), and (b) whether to advertise this best path to its neighbors (\textit{path export}). We assume that nodes follow the classic valley-free (VF) model (or, Gao-Rexford model), which guarantees the BGP routing convergence and absence of routing loops~\cite{}%
%
\footnote{The majority of routing paths in the Internet have been observed to conform to the VF model. However, as shown in \vkotronis{here cite philippa's and Giotsas's papers.} some nodes might not always follow VF-compliant policies; we discuss how to handle these cases in practice and their impact in Section.\pavlos{TODO: this sentence needs better phrasing. Think how to not over-stress it, but also not to hide that the impact in predictions can be considerable.}\vkotronis{Also we mention the same info in the footnote above, we need to keep only one.}
}%
.

\textit{Best path selection}. %In Internet routing a node $i$ receives paths for a destination from (some or all of) its neighbors and selects one of these paths as the best path. 
Under the VF model, a node prefers paths received by customers to paths from peers, and then to paths from providers (\eg $i$ prefers a path from a provider, only if it has not received any path from a customer or peer); we denote this path preference as 
\begin{equation}
customer \succ peer \succ provider
\end{equation}
If paths are learned from more than one customers (or peers/providers), then $i$ prefers the path from the customer with the highest local preference\pavlos{cite cisco best-path selection algorithm}. We denote the set of local preferences in the network as $\mathcal{Q} = \{q_{ij}\in\mathbb{R}: i,j\in\mathcal{N},e_{ij}\in\mathcal{E}\}$\footnote{We consider that a local preference is captured by a number (as, \eg in Cisco routers\pavlos{is this correct?} \vkotronis{yes, I think the footnote is redundant. Otherwise we can simply state that the higher the LP the more preferable the path is.}).}. Note that local preferences are in general asymmetric, \ie $q_{ij}\neq q_{ji}$. Since local preferences are not made public by networks, in the remainder --unless otherwise stated-- we consider that the values of local preferences are \textit{not} known \vkotronis{\emph{a priori}}.

\textit{Path export.} Moreover, under the VF model, when a node has a best path for $n_{dst}$ through a customer, it advertises this path to all its neighbors (customers/peers/providers); and when the best path is through a peer or provider, $i$ advertises this path only to its customers.

In general, VF-complying networks behave in a way that either provides them profit (e.g., routes via customers are profitable), or avoids unnecessary transit expenses (e.g., while routes via IXPs are typically settlement-free, providers get paid for transit).

\subsection{Peering Points}
Let assume a node $n_{dst}$ that originates a prefix, and is connected to its neighbors through a set of peering points $\mathcal{M}$. A peering point can be a router of the network that is used exclusively in a private peering link (\eg with its upstream provider) or a router at an IXP that connects the network to multiple other networks (the members of the IXP). 

Each neighbor $i$ of $n_{dst}$ is connected to \vkotronis{$n_{dst}$ via} exactly one peering point $m$, $m\in\mathcal{M}$, and we denote this as $i\rhd m$ \vkotronis{is the latter a strong assumption? We have discussed that there can be multiple peering points where two nodes can be connected to each other. Or do we assume node break-down in this case?}. Every other node $i$, $i\in\mathcal{N}$, selects a best path $\bestaspath{i}{n_{dst}}$ towards $n_{dst}$, \eg 
\begin{equation*}
\bestaspath{i}{n_{dst}} = [i,x,...,y,n_{dst}]
\end{equation*}
where node $x$ is a neighbor of $i$, and $y$ a neighbor of $n_{dst}$\footnote{It might happen that $\bestaspath{i}{n_{dst}} = [i,n_{dst}]$; in this case $i$ is a direct neighbor of $n_{dst}$).}. In the above example, if $y\rhd m$, $m\in\mathcal{M}$, we write also that $\bestaspath{i}{n_{dst}}\rhd m$.

We define a function (\textit{routing function}) $f:\mathcal{N}\rightarrow \mathcal{M}\cup \{0\}$ that maps nodes to peering points as follows
\begin{equation}\label{eq:routing-function}
f(i) = \left\{
\begin{tabular}{ll}
{m} & {, if $\bestaspath{i}{n_{dst}}\rhd m$}\\
{0} & {, if $\bestaspath{i}{n_{dst}}$ is not known}
\end{tabular}
\right.
\end{equation}
In other words, $f(i)=0$ denotes an uncertainty for the route of node $i$.

\pavlos{ a different definition could be this
\begin{equation}\label{eq:routing-function-new-def}
f(i) = \left\{
\begin{tabular}{ll}
{m} & {, if $Prob\{\bestaspath{i}{n_{dst}}\rhd m\}=1$}\\
{0} & {, otherwise}
\end{tabular}
\right.
\end{equation}
where
\begin{equation}
m = \arg\max_{k\in\mathcal{M}} Prob\{\bestaspath{i}{n_{dst}}\rhd k\}
\end{equation}
}

\vkotronis{@Pavlos: I like better the latter definition, although if we go into probabilistic mode I would use a threshold rather than ``1''. We can simply say that for absolute certainty we need the threshold to be 1. Also we need to explain somewhere that due to the potential uncertainty w.r.t. routing policies and local preferences we may need to resort to a probabilistic estimation of the routes between $i$ and $n_{dst}$ (and provide an example with a small graph).}


==> NFA_backup.tex <==

\pavlos{Here, a bit about the theory of NFA, and extra steps we use to reduce complexity.} 

\subsubsection{Policy-compliant Path Transform}

As stated in our basic model, the --directed-- edges $\mathcal{E}$ of graph $\mathcal{G}$ are annotated/labeled with their related VF classification ($c2p$, $p2c$, $p2p$).
Following the methodology of Kloeti \emph{et al.}~\cite{}, we express the policies corresponding to the relationship labels using regular expressions, and thus --by extension-- NFAs adhering to these expressions. Under the VF-model, all policy-compliant paths adhere to the following regular expression\footnote{Note that while in this paper we focus on valley-freeness, the NFA can be modified/extended to match any kind of policy that can be expressed via a regular expression.}: $c2p*p2p?p2c*$. 
$*$  denotes the existence of $0,1, 2, ...$ links of the type denoted left of the symbol, and $?$ denotes the existence of at most one (\ie $0$ or $1$) links of the type denoted left of the symbol. For example, a path with the following sequence of link types is VF-compliant:
\begin{equation*}
p2p - p2c - p2c
\end{equation*}
whereas the following path is not VF-compliant:
\begin{equation*}
c2p - c2p - p2c - c2p
\end{equation*}
because it contains a \textit{c2p} link after a \textit{p2c} link.

\begin{figure}
\centering
\includegraphics[width=0.5\columnwidth]{./figures/vf-nfa.eps}
\caption{Valley-free NFA. Paths
can only go first ``up'' (c2p) and then ``down'' (p2c), while
at most one p2p link can connect an ``up'' with a ``down''
transition forming a ``mountain'' with a p2p link on its ``peak''. The peak may also be sharper, with a direct transition from ``up'' to ``down''.}
\label{fig:vf-nfa}
\end{figure}

The aforementioned regular expression corresponds to the NFA (VF-NFA) shown in Fig.~\ref{fig:vf-nfa}. Our objective is to transform the original --labeled-- graph $\mathcal{G}$ into another graph $\mathcal{G'}$ such that only policy-compliant paths exist in $\mathcal{G'}$.
To achieve this, we calculate the tensor product between $G$ and the NFA transition graph $T$; $T$ comprises a node set consisting of the states of the VF-NFA, and an edge set consisting of all permitted state transitions between the nodes.
Thus $T=(\mathcal{Q}, \Delta)$, where\footnote{For brevity, we skip the full definition of NFA terminating and starting states, as well as other redundant details which can be found in~\cite{}.}:\\
$\mathcal{Q}=\{up,down\}$ is the set of NFA states, and\\ $\Delta=\cup_{s}{\Delta_{s}}$ is the union of the sets of NFA transitions related to symbol/label $s$. Therefore:\\
$\Delta_{c2p} = \{up\rightarrow{up}\}$\\
$\Delta_{p2p} = \{up\rightarrow{down}\}$\\
$\Delta_{p2c} = \{up\rightarrow{down},down\rightarrow{down}\}$\\
For each of the relationship symbols $s \in \{c2p,p2p,p2c\}$, we form the subgraphs $G_s$ and $T_s$ consisting
of all the edges labeled with $s$. We then form the \emph{tensor product} of these
subgraphs, which is defined as follows: if $v_1$ and $v_2$ are nodes in $G$ and $q_1$ and
$q_2$ are nodes in $T$, then $G'$ contains the nodes $(v_1,q_1)$, $(v_1,q_2)$, $(v_2,q_1)$
and $(v_2,q_2)$. Likewise, if there is an edge $(v_1,v_2)$ in the subgraph $G_s$ and an
edge $(q_1,q_2)$ in the subgraph $T_s$, then the tensor product contains the edge
$((v_1,q_1),(v_2,q_2))$. The union of all of these tensor products is the transformed graph $G'$. Examples of the application of tensor products on VF-labeled links are given in Fig.~\ref{fig:vft-examples}. As proven in~\cite{}, $G'$ contains only (and all possible) policy-compliant paths between any pair of nodes, conforming to the VF-model. Since $G'$ is not labeled --thus not requiring special handling of policies--, we can run off-the-self algorithms for path calculation without any policy-specific modifications.
%\footnote{Note that in contrast to~\cite{}, we are not interested in min-cut calculations, but only in node-to-node path calculations. Therefore, we defer from adding more complexity with extra aggregation states to the transformation process.}.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{./figures/vft-examples.eps}
\caption{Examples of graph link transformations. Nodes are divided in two state nodes, while labeled links are transformed to unlabeled state transitions.}
\label{fig:vft-examples}
\end{figure}

% Given the node relationships, we can directly tell whether a path is VF-compliant. The sequence of links in a VF-compliant paths can be of the following types:
% \begin{equation}
% (c2p)* - (p2p)? - (p2c)* 
% \end{equation}
% where $*$  denotes the existence of $0,1, 2, ...$ links of the type denoted in the parenthesis, and $?$ denotes the existence of at most one (\ie $0$ or $1$) paths of the type denoted in the parenthesis. For example, a path with the following sequence of link types is VF-compliant
% \begin{equation*}
% p2p - p2c - p2c
% \end{equation*}
% whereas the following path is not VF-compliant
% \begin{equation*}
% c2p - c2p - p2c - c2p
% \end{equation*}
% because it contains a \textit{c2p} link after a \textit{p2c} link. 

The spatial complexity of the transformed graph $\mathcal{G'}$ is\footnote{Note that in contrast to~\cite{}, which involves a more complex graph transform with aggregation states and $\epsilon$-transitions (for preserving min-cuts), we focus on the --simpler-- objective of solely policy-compliant path calculation. This affects our spatial and temporal complexity results, which are actually reduced.}:
\begin{equation}
|\mathcal{N}'| = \mathcal{O}(|\mathcal{N}|\cdot|\mathcal{Q}|)
\end{equation}
in terms of nodes, and:
\begin{equation}
|\mathcal{E}'| = \mathcal{O}(|\mathcal{E}|\cdot{max_{s}}(|\Delta_{s}|))
\end{equation}
in terms of edges.

The temporal complexity for the generation of the transformed graph is:
\begin{equation}
t_{gen}=\mathcal{O}(|\mathcal{N}|\cdot|\mathcal{Q}| + |\mathcal{E}|\cdot{max_{s}}(|\Delta_{s}|))
\end{equation}

To calculate all acyclic paths between a pair of nodes in a graph $\mathcal{G}$ is of --high-- computational complexity $O(\mathcal{N}!)$. Doing this for every node $j\in\mathcal{N}$ to node $i$, in a simple implementation is of complexity $O(\mathcal{N}!\cdot \mathcal{N})$.
\pavlos{check if these two arguments above are correct}. 
\vkotronis{yes, they seem correct.}
%To reduce this complexity we follow the approach of~\red{[NFA-paper]}.
In order to reduce this complexity, which is even higher for the transformed graph $\mathcal{G}'$ which has double the number of nodes and in the worst case double the number of edges of the initial graph $\mathcal{G}$, we go through the following steps: \pavlos{describe the steps of the method}
\begin{enumerate}
\item \vkotronis{Prune all ``stub'' nodes (and corresponding edges) from $\mathcal{G}$, i.e., nodes that are only related via a $c2p$ link to another node and all their paths (i.e., paths involving them as source or destination) pass through this node (i.e., single upstream case). To reduce the size of the node and edge sets, we can represent the behavior of these nodes via their upstreams, and reinstate them at the end of our calculations without any loss of generality.}
\item Transform graph $\mathcal{G}$ to $\mathcal{G}'$, using the VF-NFA (as analyzed previously).
\item Do a DFS search from the node $i$ to every other node $j$
% \vkotronis{@Pavlos: Could you explain the exact process you follow for the path calculation? I do not remember exactly the trick, but I think you generate all possible preferred policy-compliant paths using selective DFS (e.g., select only customers if available, peers if customers not available, providers if peers or customers not available, etc.)}
\end{enumerate}
% \pavlos{correctness of the method?  + complexity?} This process satisfies that all the VF-compliant paths are found \pavlos{?}. 
\vkotronis{@Pavlos: Actually calculating all paths is not computationally tractable, so we proceed directly to the sDFS!
Could you bridge this a bit better?}

\subsection{Step 2 - Calculate Best VF-paths}
Instead of calculating all the VF-compliant paths from $j$ to $i$ on the transformed graph, which is a computationally intractable task, we instead infer which of them are finally selected by $j$ as the ``best'' paths. To this end, we can use the path ordering rules, to eliminate paths. For instance, if there are two VF-compliant paths from $j$ to $i$:
\begin{equation*}
path1 = [j,x,...,i]~~~~path2 = [j,y,...,i]
\end{equation*}
and the links $e_{jx}$ and $e_{jy}$ are \textit{p2c} and \textit{c2p}, then $j$ will prefer the path from its customer $x$ rather than its provider $y$, \ie $path1\succ path2$, and $path1$ will be the best path.

However, directly applying the path ordering rule to all the VF-paths of an arbitrary node $j$ might lead to wrong inferences, because some of these paths might never reach the node $j$. Consider the example of Fig.~\ref{fig:example-all-vf-paths}, where the VF-paths from node $i$ to $i$ are the following
\begin{align*}
path1 &= [i,x1,z,x,w,j]\\
path2 &= [i,x1,z,y,j]\\
path3 &= [i,y1,z,x,w,j]
\end{align*}
Node $i$ receives paths from its providers $x1$ and $y1$; this paths are of equivalent type, and let node $i$ prefer the shorter paths. Then, applying directly the ordering on all the VF-paths the paths of node $i$ would give
\begin{equation*}
path2 \succeq path3=path1
\end{equation*}
and $path2$ would be preferred. However, the VF-paths for $z$ (to $j$) are
\begin{align*}
path4 &= [z,x,w,j]\\
path5 &= [z,y,j]
\end{align*}
and it holds that $path4 \succ path5$. Thus, node $z$ selects as its best path $path_{zj}$ the $path4$ and this is the only paths that advertises to its neighbors $x1$ and $y1$. As a result, node $i$, receives only the paths $path1$ and $path3$, and would not receive $path2$, \ie not all VF-paths are received by a node. Hence, we need a method that first calculates the best paths for the nodes that are ``closer'' to the destination node, and then for ``farther'' nodes.
% \begin{equation*}
% path1 = [j,x,...,z,x1,...,i]~~~~path2 = [j,y,...,z,y1...,i]
% \end{equation*}
% for which it holds that $path1\succ path2$ because $j$ prefers paths from $x$ rather than $y$. However, both paths have as an intermediate hop the node $z$. Let assume that node $z$ selects its best path $path_{zi}$ between the two VF-paths
% \begin{equation*}
% path3 = [z,x1,...,i]~~~~path4 = [z,y1...,i]
% \end{equation*}
% and, due to the relationships of node $z$, it holds that $path4\succ path3$. Then, $z$ will advertise to its neighbors only the $path4$. In this case, node $j$ will never receive the $path1$, and will select as its best path, the $path2$.

To this end, we design Algorithm~\ref{alg:all-vf-paths} that calculates all eligible VF-paths (\ie discarding the VF-paths that are ``strictly smaller''), from every node $i\in\mathcal{N}$ to a node $j$. \pavlos{ADD here the description of the algorithm} \vkotronis{done, please check} \vkotronis{We also need to check together if algorithm 1 can be optimized a bit, but it seems correct.}

\myitem{Input.} Algorithm~\ref{alg:all-vf-paths} receives as input:
\begin{itemize}
\item $\mathcal{G}$: the network graph (transformed via the tensor product of the original graph and the NFA, calculated during the previous step), containing the set of nodes $\mathcal{N}$, and the set of edges $\mathcal{E}$.
\item $j$: destination node $\in{\mathcal{N}}$
\end{itemize}

\myitem{Output.} Algorithm~\ref{alg:all-vf-paths} returns as output:

\begin{itemize}
\item $\mathcal{P}$: set of all VF eligible/preferred paths from all nodes to destination $j$.
\end{itemize}

\myitem{Workflow.} Algorithm~\ref{alg:all-vf-paths} iterates over all nodes of the graph as sources\footnote{Note that since in the VF case, the transformed graph replaces each of the original nodes with 2 subnodes (e.g., node $i$ is actually split in $i_{up}$ and $i_{down}$, same with $j$), we actually use virtual sources and destinations connected directly to their respective subnode pairs; for the rest of the description though we use the notation $i$ and $j$ for the source and destination for simplicity.} (except for the destination) and gradually builds the set of admissible paths connecting these sources with the destination (\emph{lines 2-7}). The knowledge of previously calculated paths (between other --potentially intermediate-- nodes and the destination) is updated and accumulated over consecutive runs of the selective DFS step (\emph{line 4}; see \emph{line 17} w.r.t.~the recursion attestation). This step receives as input a source-destination node pair, the set of graph edges and the already calculated path set (\emph{line 8}). Then, it scans all neighbors (\emph{lines 10-11}) of the source in terms of available paths, in a \textit{specific order} (first customers, then peers, then providers; \emph{line 10}), so that VF preference is respected until the destination is reached (\emph{lines 12-14}). This process is performed in a recursive DFS manner (\emph{lines 16-18}), with the partial paths to and from the neighbors of each explored node being eventually stitched together to form e2e paths to the destination (\emph{lines 20-22}). Note that as described before, the order of exploration is aligned to the VF preference; if a currently explored class of the neighbors of a specific node (e.g., customers) has at least one valid path to the destination\footnote{Note that paths can contain several class transitions e2e, e.g., $c2p-p2p-p2c$; here we are looking at path exploration from the local perspective of the currently explored node.}, its exploration continues in order to yield the full possible set related to this class (\emph{lines 11-25}), but it does not proceed to the next class (\emph{lines 26-27}). The latter happens only in the case the currently explored class does not yield any paths. This guarantees that we only explore DFS paths that are actually \textit{preferred} by the nodes based on their local preference of the next hop in the path\footnote{We remind the reader that the transformed graph already transforms --only-- all possible VF paths, preferred or not.} and drastically reduces the complexity of a --potential naive-- full DFS exploration. We remind the reader that these paths always contain the actually best path, which can be selected per node for the respective class (e.g., customers) based on weak path ordering (using, for example, the path length as the tie-breaker).

\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{./figures/example_all_vf-paths.eps}
\caption{Example. Directed edges denote a \textit{c2p} relationship (pointing to the provider), and edges with double arrows denote a \textit{p2p} relationship.}
\label{fig:example-all-vf-paths}
\end{figure}

\begin{algorithm}[t]%[h]
\caption{Calculate all eligible VF-paths to destination.}
\label{alg:all-vf-paths}
\begin{small}
\begin{algorithmic}[1]
% input:
\Statex {\textbf{Input:} NFA network graph $\mathcal{G}(\mathcal{N},\mathcal{E})$; destination node $j$.}
% main algorithm:
\State $\mathcal{P}\leftarrow \emptyset$  \Comment set of all VF-paths to $j$
\For {$i\in\mathcal{N}\backslash\{j\}$}
	\If {\textproc{get\_paths}($i,j,\mathcal{P}$)$=\emptyset$}
    	\State $\mathcal{P}\leftarrow \mathcal{P}~\cup$~\textproc{selectiveDFS}($i,j,\mathcal{E},\mathcal{P}$)
    \EndIf
\EndFor
\State\Return $\mathcal{P}$

% sub-routine "selectiveDFS"
\Statex {}
\Function{selectiveDFS}{$i,j,\mathcal{E},\mathcal{P}$}
\State $P_{i,j}\leftarrow \emptyset$  \Comment set of all VF-paths from $i$ to $j$
\For {$N_{i} \in [\mathcal{C}_{i}, \mathcal{P}_{i}, \mathcal{U}_{i}]$}
	\For {$k\in N_{i}$}
    	\If {$k=j$}
        	\State $current\_path \leftarrow [i,j]$
            \State $\mathcal{P}\leftarrow \mathcal{P}~\cup~\{current\_path\}$
        \Else 
        	\If {\textproc{get\_paths}($k,j,\mathcal{P}$)$=\emptyset$}
            	\State $\mathcal{P}\leftarrow \mathcal{P}~\cup$~\textproc{selectiveDFS}($k,j,\mathcal{E},\mathcal{P}$)
            \EndIf
			\State $P_{k,j}\leftarrow$ \textproc{get\_paths}($k,j,\mathcal{P}$)
            \For {$path_{kj}\in P_{k,j}$}
            	\State $current\_path \leftarrow [i,path_{kj}]$
            	\State $P_{i,j}\leftarrow P_{i,j}~\cup~\{current\_path\}$
            \EndFor
        \EndIf
    \EndFor
    \If {$P_{i,j} \neq \emptyset$}
    	\State \Break    	
    \EndIf
\EndFor
\State $\mathcal{P}\leftarrow \mathcal{P} \cup P_{i,j}$ 
\State \Return $\mathcal{P}$
\EndFunction

% sub-routine "get_paths"
\Statex {}
\Function{get\_paths}{$i,j,\mathcal{P}$} 
\State $P_{i,j}\leftarrow\{path\in\mathcal{P}: path_{src}=i,~path_{dst}=j\}$
\State \Return $P_{i,j}$
\EndFunction
\end{algorithmic}
\end{small}
\end{algorithm}

==> PathInference_backup.tex <==
We consider a network with known nodes $\mathcal{N}$, edges $\mathcal{E}$, and \vkotronis{corresponding} node relationships \vkotronis{should we also baptize the set of relationships or do we consider them as simple annotations of the link as in the previous section?}. Let us assume that a node $i$ advertises a prefix $pfx_{i}$, and that each node $j$, $j\in\mathcal{N}$, has a best path $path_{ji}$, \eg
\begin{equation}
path_{ji} = [j,x,...,y,i]
\end{equation}
where node $x$ is a neighbor of $j$, and node $y$ a neighbor of $i$ (it might happen that $path_{ji} = [j,i]$; in this case $j$ is a direct neighbor of $i$).
\vkotronis{again, I think that we should revisit the path definition since the destination node is not so important if it is not a direct neighbor of the source; the prefix is the end-goal of routing.}

\myitem{The problem.} Our goal is to infer which of all possible paths from $j$ to $i$ is the best path $path_{ji}$. Or, we might only want to know which is the peering point through which $i$ is reached (\ie which is the last hop before node $i$), \eg in the above example the node $y$. \vkotronis{We need to justify the latter sub-problem/objective.}

\myitem{Methodology overview.} We answer the above question by using a methodology that is summarized in the following two steps: (i) we first calculate for every node $j\in\mathcal{N}$ all its \textit{eligible} (\ie conforming to the routing model; here, the VF-model) paths to node $i$, and then (ii) we calculate which of all the eligible paths of node $j$ is the best path $path_{ji}$, based on the (strict/weak) path ordering.

We now present in detail, the steps of the methodology, and discuss the related challenges.

\subsection{Step 1 - Calculate all VF paths.} 

\pavlos{Here, a bit about the theory of NFA, and extra steps we use to reduce complexity.} 

\subsubsection{Policy-compliant Path Transform}

As stated in our basic model, the --directed-- edges $\mathcal{E}$ of graph $\mathcal{G}$ are annotated/labeled with their related VF classification ($c2p$, $p2c$, $p2p$).
Following the methodology of Kloeti \emph{et al.}~\cite{}, we express the policies corresponding to the relationship labels using regular expressions, and thus --by extension-- NFAs adhering to these expressions. Under the VF-model, all policy-compliant paths adhere to the following regular expression\footnote{Note that while in this paper we focus on valley-freeness, the NFA can be modified/extended to match any kind of policy that can be expressed via a regular expression.}: $c2p*p2p?p2c*$. 
$*$  denotes the existence of $0,1, 2, ...$ links of the type denoted left of the symbol, and $?$ denotes the existence of at most one (\ie $0$ or $1$) links of the type denoted left of the symbol. For example, a path with the following sequence of link types is VF-compliant:
\begin{equation*}
p2p - p2c - p2c
\end{equation*}
whereas the following path is not VF-compliant:
\begin{equation*}
c2p - c2p - p2c - c2p
\end{equation*}
because it contains a \textit{c2p} link after a \textit{p2c} link.

\begin{figure}
\centering
\includegraphics[width=0.5\columnwidth]{./figures/vf-nfa.eps}
\caption{Valley-free NFA. Paths
can only go first ``up'' (c2p) and then ``down'' (p2c), while
at most one p2p link can connect an ``up'' with a ``down''
transition forming a ``mountain'' with a p2p link on its ``peak''. The peak may also be sharper, with a direct transition from ``up'' to ``down''.}
\label{fig:vf-nfa}
\end{figure}

The aforementioned regular expression corresponds to the NFA (VF-NFA) shown in Fig.~\ref{fig:vf-nfa}. Our objective is to transform the original --labeled-- graph $\mathcal{G}$ into another graph $\mathcal{G'}$ such that only policy-compliant paths exist in $\mathcal{G'}$.
To achieve this, we calculate the tensor product between $G$ and the NFA transition graph $T$; $T$ comprises a node set consisting of the states of the VF-NFA, and an edge set consisting of all permitted state transitions between the nodes.
Thus $T=(\mathcal{Q}, \Delta)$, where\footnote{For brevity, we skip the full definition of NFA terminating and starting states, as well as other redundant details which can be found in~\cite{}.}:\\
$\mathcal{Q}=\{up,down\}$ is the set of NFA states, and\\ $\Delta=\cup_{s}{\Delta_{s}}$ is the union of the sets of NFA transitions related to symbol/label $s$. Therefore:\\
$\Delta_{c2p} = \{up\rightarrow{up}\}$\\
$\Delta_{p2p} = \{up\rightarrow{down}\}$\\
$\Delta_{p2c} = \{up\rightarrow{down},down\rightarrow{down}\}$\\
For each of the relationship symbols $s \in \{c2p,p2p,p2c\}$, we form the subgraphs $G_s$ and $T_s$ consisting
of all the edges labeled with $s$. We then form the \emph{tensor product} of these
subgraphs, which is defined as follows: if $v_1$ and $v_2$ are nodes in $G$ and $q_1$ and
$q_2$ are nodes in $T$, then $G'$ contains the nodes $(v_1,q_1)$, $(v_1,q_2)$, $(v_2,q_1)$
and $(v_2,q_2)$. Likewise, if there is an edge $(v_1,v_2)$ in the subgraph $G_s$ and an
edge $(q_1,q_2)$ in the subgraph $T_s$, then the tensor product contains the edge
$((v_1,q_1),(v_2,q_2))$. The union of all of these tensor products is the transformed graph $G'$. Examples of the application of tensor products on VF-labeled links are given in Fig.~\ref{fig:vft-examples}. As proven in~\cite{}, $G'$ contains only (and all possible) policy-compliant paths between any pair of nodes, conforming to the VF-model. Since $G'$ is not labeled --thus not requiring special handling of policies--, we can run off-the-self algorithms for path calculation without any policy-specific modifications.
%\footnote{Note that in contrast to~\cite{}, we are not interested in min-cut calculations, but only in node-to-node path calculations. Therefore, we defer from adding more complexity with extra aggregation states to the transformation process.}.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{./figures/vft-examples.eps}
\caption{Examples of graph link transformations. Nodes are divided in two state nodes, while labeled links are transformed to unlabeled state transitions.}
\label{fig:vft-examples}
\end{figure}

% Given the node relationships, we can directly tell whether a path is VF-compliant. The sequence of links in a VF-compliant paths can be of the following types:
% \begin{equation}
% (c2p)* - (p2p)? - (p2c)* 
% \end{equation}
% where $*$  denotes the existence of $0,1, 2, ...$ links of the type denoted in the parenthesis, and $?$ denotes the existence of at most one (\ie $0$ or $1$) paths of the type denoted in the parenthesis. For example, a path with the following sequence of link types is VF-compliant
% \begin{equation*}
% p2p - p2c - p2c
% \end{equation*}
% whereas the following path is not VF-compliant
% \begin{equation*}
% c2p - c2p - p2c - c2p
% \end{equation*}
% because it contains a \textit{c2p} link after a \textit{p2c} link. 

The spatial complexity of the transformed graph $\mathcal{G'}$ is\footnote{Note that in contrast to~\cite{}, which involves a more complex graph transform with aggregation states and $\epsilon$-transitions (for preserving min-cuts), we focus on the --simpler-- objective of solely policy-compliant path calculation. This affects our spatial and temporal complexity results, which are actually reduced.}:
\begin{equation}
|\mathcal{N}'| = \mathcal{O}(|\mathcal{N}|\cdot|\mathcal{Q}|)
\end{equation}
in terms of nodes, and:
\begin{equation}
|\mathcal{E}'| = \mathcal{O}(|\mathcal{E}|\cdot{max_{s}}(|\Delta_{s}|))
\end{equation}
in terms of edges.

The temporal complexity for the generation of the transformed graph is:
\begin{equation}
t_{gen}=\mathcal{O}(|\mathcal{N}|\cdot|\mathcal{Q}| + |\mathcal{E}|\cdot{max_{s}}(|\Delta_{s}|))
\end{equation}

To calculate all acyclic paths between a pair of nodes in a graph $\mathcal{G}$ is of --high-- computational complexity $O(\mathcal{N}!)$. Doing this for every node $j\in\mathcal{N}$ to node $i$, in a simple implementation is of complexity $O(\mathcal{N}!\cdot \mathcal{N})$.
\pavlos{check if these two arguments above are correct}. 
\vkotronis{yes, they seem correct.}
%To reduce this complexity we follow the approach of~\red{[NFA-paper]}.
In order to reduce this complexity, which is even higher for the transformed graph $\mathcal{G}'$ which has double the number of nodes and in the worst case double the number of edges of the initial graph $\mathcal{G}$, we go through the following steps: \pavlos{describe the steps of the method}
\begin{enumerate}
\item \vkotronis{Prune all ``stub'' nodes (and corresponding edges) from $\mathcal{G}$, i.e., nodes that are only related via a $c2p$ link to another node and all their paths (i.e., paths involving them as source or destination) pass through this node (i.e., single upstream case). To reduce the size of the node and edge sets, we can represent the behavior of these nodes via their upstreams, and reinstate them at the end of our calculations without any loss of generality.}
\item Transform graph $\mathcal{G}$ to $\mathcal{G}'$, using the VF-NFA (as analyzed previously).
\item Do a DFS search from the node $i$ to every other node $j$
% \vkotronis{@Pavlos: Could you explain the exact process you follow for the path calculation? I do not remember exactly the trick, but I think you generate all possible preferred policy-compliant paths using selective DFS (e.g., select only customers if available, peers if customers not available, providers if peers or customers not available, etc.)}
\end{enumerate}
% \pavlos{correctness of the method?  + complexity?} This process satisfies that all the VF-compliant paths are found \pavlos{?}. 
\vkotronis{@Pavlos: Actually calculating all paths is not computationally tractable, so we proceed directly to the sDFS!
Could you bridge this a bit better?}

\subsection{Step 2 - Calculate Best VF-paths}
Instead of calculating all the VF-compliant paths from $j$ to $i$ on the transformed graph, which is a computationally intractable task, we instead infer which of them are finally selected by $j$ as the ``best'' paths. To this end, we can use the path ordering rules, to eliminate paths. For instance, if there are two VF-compliant paths from $j$ to $i$:
\begin{equation*}
path1 = [j,x,...,i]~~~~path2 = [j,y,...,i]
\end{equation*}
and the links $e_{jx}$ and $e_{jy}$ are \textit{p2c} and \textit{c2p}, then $j$ will prefer the path from its customer $x$ rather than its provider $y$, \ie $path1\succ path2$, and $path1$ will be the best path.

However, directly applying the path ordering rule to all the VF-paths of an arbitrary node $j$ might lead to wrong inferences, because some of these paths might never reach the node $j$. Consider the example of Fig.~\ref{fig:example-all-vf-paths}, where the VF-paths from node $i$ to $i$ are the following
\begin{align*}
path1 &= [i,x1,z,x,w,j]\\
path2 &= [i,x1,z,y,j]\\
path3 &= [i,y1,z,x,w,j]
\end{align*}
Node $i$ receives paths from its providers $x1$ and $y1$; this paths are of equivalent type, and let node $i$ prefer the shorter paths. Then, applying directly the ordering on all the VF-paths the paths of node $i$ would give
\begin{equation*}
path2 \succeq path3=path1
\end{equation*}
and $path2$ would be preferred. However, the VF-paths for $z$ (to $j$) are
\begin{align*}
path4 &= [z,x,w,j]\\
path5 &= [z,y,j]
\end{align*}
and it holds that $path4 \succ path5$. Thus, node $z$ selects as its best path $path_{zj}$ the $path4$ and this is the only paths that advertises to its neighbors $x1$ and $y1$. As a result, node $i$, receives only the paths $path1$ and $path3$, and would not receive $path2$, \ie not all VF-paths are received by a node. Hence, we need a method that first calculates the best paths for the nodes that are ``closer'' to the destination node, and then for ``farther'' nodes.
% \begin{equation*}
% path1 = [j,x,...,z,x1,...,i]~~~~path2 = [j,y,...,z,y1...,i]
% \end{equation*}
% for which it holds that $path1\succ path2$ because $j$ prefers paths from $x$ rather than $y$. However, both paths have as an intermediate hop the node $z$. Let assume that node $z$ selects its best path $path_{zi}$ between the two VF-paths
% \begin{equation*}
% path3 = [z,x1,...,i]~~~~path4 = [z,y1...,i]
% \end{equation*}
% and, due to the relationships of node $z$, it holds that $path4\succ path3$. Then, $z$ will advertise to its neighbors only the $path4$. In this case, node $j$ will never receive the $path1$, and will select as its best path, the $path2$.

To this end, we design Algorithm~\ref{alg:all-vf-paths} that calculates all eligible VF-paths (\ie discarding the VF-paths that are ``strictly smaller''), from every node $i\in\mathcal{N}$ to a node $j$. \pavlos{ADD here the description of the algorithm} \vkotronis{done, please check} \vkotronis{We also need to check together if algorithm 1 can be optimized a bit, but it seems correct.}

\myitem{Input.} Algorithm~\ref{alg:all-vf-paths} receives as input:
\begin{itemize}
\item $\mathcal{G}$: the network graph (transformed via the tensor product of the original graph and the NFA, calculated during the previous step), containing the set of nodes $\mathcal{N}$, and the set of edges $\mathcal{E}$.
\item $j$: destination node $\in{\mathcal{N}}$
\end{itemize}

\myitem{Output.} Algorithm~\ref{alg:all-vf-paths} returns as output:

\begin{itemize}
\item $\mathcal{P}$: set of all VF eligible/preferred paths from all nodes to destination $j$.
\end{itemize}

\myitem{Workflow.} Algorithm~\ref{alg:all-vf-paths} iterates over all nodes of the graph as sources\footnote{Note that since in the VF case, the transformed graph replaces each of the original nodes with 2 subnodes (e.g., node $i$ is actually split in $i_{up}$ and $i_{down}$, same with $j$), we actually use virtual sources and destinations connected directly to their respective subnode pairs; for the rest of the description though we use the notation $i$ and $j$ for the source and destination for simplicity.} (except for the destination) and gradually builds the set of admissible paths connecting these sources with the destination (\emph{lines 2-7}). The knowledge of previously calculated paths (between other --potentially intermediate-- nodes and the destination) is updated and accumulated over consecutive runs of the selective DFS step (\emph{line 4}; see \emph{line 17} w.r.t.~the recursion attestation). This step receives as input a source-destination node pair, the set of graph edges and the already calculated path set (\emph{line 8}). Then, it scans all neighbors (\emph{lines 10-11}) of the source in terms of available paths, in a \textit{specific order} (first customers, then peers, then providers; \emph{line 10}), so that VF preference is respected until the destination is reached (\emph{lines 12-14}). This process is performed in a recursive DFS manner (\emph{lines 16-18}), with the partial paths to and from the neighbors of each explored node being eventually stitched together to form e2e paths to the destination (\emph{lines 20-22}). Note that as described before, the order of exploration is aligned to the VF preference; if a currently explored class of the neighbors of a specific node (e.g., customers) has at least one valid path to the destination\footnote{Note that paths can contain several class transitions e2e, e.g., $c2p-p2p-p2c$; here we are looking at path exploration from the local perspective of the currently explored node.}, its exploration continues in order to yield the full possible set related to this class (\emph{lines 11-25}), but it does not proceed to the next class (\emph{lines 26-27}). The latter happens only in the case the currently explored class does not yield any paths. This guarantees that we only explore DFS paths that are actually \textit{preferred} by the nodes based on their local preference of the next hop in the path\footnote{We remind the reader that the transformed graph already transforms --only-- all possible VF paths, preferred or not.} and drastically reduces the complexity of a --potential naive-- full DFS exploration. We remind the reader that these paths always contain the actually best path, which can be selected per node for the respective class (e.g., customers) based on weak path ordering (using, for example, the path length as the tie-breaker).

\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{./figures/example_all_vf-paths.eps}
\caption{Example. Directed edges denote a \textit{c2p} relationship (pointing to the provider), and edges with double arrows denote a \textit{p2p} relationship.}
\label{fig:example-all-vf-paths}
\end{figure}

\begin{algorithm}[t]%[h]
\caption{Calculate all eligible VF-paths to destination.}
\label{alg:all-vf-paths}
\begin{small}
\begin{algorithmic}[1]
% input:
\Statex {\textbf{Input:} NFA network graph $\mathcal{G}(\mathcal{N},\mathcal{E})$; destination node $j$.}
% main algorithm:
\State $\mathcal{P}\leftarrow \emptyset$  \Comment set of all VF-paths to $j$
\For {$i\in\mathcal{N}\backslash\{j\}$}
	\If {\textproc{get\_paths}($i,j,\mathcal{P}$)$=\emptyset$}
    	\State $\mathcal{P}\leftarrow \mathcal{P}~\cup$~\textproc{selectiveDFS}($i,j,\mathcal{E},\mathcal{P}$)
    \EndIf
\EndFor
\State\Return $\mathcal{P}$

% sub-routine "selectiveDFS"
\Statex {}
\Function{selectiveDFS}{$i,j,\mathcal{E},\mathcal{P}$}
\State $P_{i,j}\leftarrow \emptyset$  \Comment set of all VF-paths from $i$ to $j$
\For {$N_{i} \in [\mathcal{C}_{i}, \mathcal{P}_{i}, \mathcal{U}_{i}]$}
	\For {$k\in N_{i}$}
    	\If {$k=j$}
        	\State $current\_path \leftarrow [i,j]$
            \State $\mathcal{P}\leftarrow \mathcal{P}~\cup~\{current\_path\}$
        \Else 
        	\If {\textproc{get\_paths}($k,j,\mathcal{P}$)$=\emptyset$}
            	\State $\mathcal{P}\leftarrow \mathcal{P}~\cup$~\textproc{selectiveDFS}($k,j,\mathcal{E},\mathcal{P}$)
            \EndIf
			\State $P_{k,j}\leftarrow$ \textproc{get\_paths}($k,j,\mathcal{P}$)
            \For {$path_{kj}\in P_{k,j}$}
            	\State $current\_path \leftarrow [i,path_{kj}]$
            	\State $P_{i,j}\leftarrow P_{i,j}~\cup~\{current\_path\}$
            \EndFor
        \EndIf
    \EndFor
    \If {$P_{i,j} \neq \emptyset$}
    	\State \Break    	
    \EndIf
\EndFor
\State $\mathcal{P}\leftarrow \mathcal{P} \cup P_{i,j}$ 
\State \Return $\mathcal{P}$
\EndFunction

% sub-routine "get_paths"
\Statex {}
\Function{get\_paths}{$i,j,\mathcal{P}$} 
\State $P_{i,j}\leftarrow\{path\in\mathcal{P}: path_{src}=i,~path_{dst}=j\}$
\State \Return $P_{i,j}$
\EndFunction
\end{algorithmic}
\end{small}
\end{algorithm}

\subsection{Step 3 - Build the VF Bayesian Network (VF-BN)}
From the paths calculated in the previous step, we build a Bayesian Network (BN) to encode all the eligible VF-paths; we refer to it as the VF- Bayesian network (VF-BN). 

A BN is a Directed Acyclic Graph (DAG), where a directed edge $e_{ij}$ denotes a dependence of the node  $j$ (end of the arrow) on the node $i$. In our case, this dependence corresponds to the routing paths \vkotronis{selected based on the routing policies of the involved nodes as well as other mechanisms of the routing protocol of choice; e.g., BGP in the AS-level Internet}. For example, an edge $e_{ij}$ denotes that the routing decision of $j$ depends on the decision of $i$, or, in other words, the path that is selected by $j$ contains as the previous hop the node $i$, and is dependent of the path selected by $i$, \ie $path_{ik} = [i,path_{jk}]$. \vkotronis{I think it should be: $path_{jk} = [i,path_{ik}]$. However, besides this correction, I am not sure that the use of ``\ie{}'' is correct here; $j$ may have various dependencies from other neighbors, does not mean that $i$ is the actual best hop right? When $i$ is the actual next hop though, you are right. What matters more IMHO is that the dependence stems from the fact that $j$ receives what $i$ exports to it, and cannot change the path of $i$ to $k$ (it can decide whether to use an alternative by invoking another dependency though).}

We use Algorithm~\ref{alg:build-vf-bn} to build the VF-BN. \pavlos{ADD description of the algorithm.} \vkotronis{done, please check}

\myitem{Input.} Algorithm~\ref{alg:build-vf-bn} receives as input: 
\begin{itemize}
\item $\mathcal{G}$: the network graph (transformed via the tensor product of the original graph and the NFA, calculated during the Step B), containing the set of nodes $\mathcal{N}$, and the set of edges $\mathcal{E}$.
\item $\mathcal{P}$: all eligible VF-paths towards a certain destination $j$ generated by Algorithm~\ref{alg:all-vf-paths}. 
\end{itemize}

\myitem{Output.} Algorithm~\ref{alg:build-vf-bn} returns as output:
\begin{itemize}
\item $\mathcal{BN}$: the Bayesian network, as a DAG rooted in node $j$ which is the termination point of all paths $\in\mathcal{P}$.
\end{itemize}

\myitem{Workflow.} Algorithm~\ref{alg:build-vf-bn}, after integrating all nodes of the input graph (\emph{line 2}), simply iterates over all calculated paths and builds the set of edges by integrating the edges forming these paths (\emph{lines 3-6}). These in-path edges correspond to the node-to-node dependencies depicted in the Bayesian network, since they stem from the actual routing policies of the involved nodes (applied in sequence to reach destination node $j$).

\vkotronis{To help the rest of the argumentation, I would recommend also including (and proving) the following Lemma (please check proof):
\begin{lemma}
Algorithm~\ref{alg:all-vf-paths} calculates all eligible VF-paths from every node $i$ to destination $j$.
\end{lemma}
\begin{proof}
Assume a path generated by Algorithm~\ref{alg:all-vf-paths} between node $i$ and $j$. Following the workflow of Algorithm~\ref{alg:all-vf-paths}, since VF preference is enforced through the strict ordering of the DFS path exploration process (prefer customers first, then peers, then providers), and the transformed graph already contains only (and all possible) --preferred or not-- VF paths, the calculated VF-paths can be only eligible (preferred) VF-paths. Moreover, since the entire graph is explored via DFS, all eligible VF-paths from every node $i$ to destination $j$ are calculated.
\end{proof}
}

\begin{lemma}
Every eligible VF-path from $i$ to $j$, can be constructed by following a sequence of directed edges, starting from $j$, in the $\mathcal{BN}$ graph.
\end{lemma}
\begin{proof}
\vkotronis{Since all nodes $\mathcal{N_{BN}}$ and edges $\mathcal{E_{BN}}$ have been used for the formation of $\mathcal{BN}$ in the same sequence as the one with which they appear on the eligible VF-paths generated by Algorithm~\ref{alg:all-vf-paths}  (see previous Lemma), $BN$ encodes eligible VF-paths towards destination $j$, albeit in the reverse direction with $j$ as a source.
Since the formation of the $\mathcal{BN}$ takes into account \textit{all} eligible-VF paths, every eligible VF-path from $i$ to $j$ can be constructed by following a sequence of directed edges (in the reverse direction), starting from $j$, in $\mathcal{BN}$.}

\end{proof}
\begin{lemma}
Every feasible path in the $\mathcal{BN}$ graph, is a VF-path.
\end{lemma}
\begin{proof}
\pavlos{TO PROVE (use the fact that every incoming edge to a node is of the same type c2p / p2p / p2c)} \vkotronis{not sure about this, I have followed a slightly different logic albeit with the same end result.}\\
\vkotronis{Since all nodes $\mathcal{N_{BN}}$ and edges $\mathcal{E_{BN}}$ have been used for the formation of $\mathcal{BN}$ in the same sequence as the one with which they appear on the eligible VF-paths generated by Algorithm~\ref{alg:all-vf-paths}  (see previous Lemma), $BN$ encodes eligible VF-paths towards destination $j$. Since Algorithm~\ref{alg:all-vf-paths} explores only VF paths on the transformed graph, and there is 1-to-1 mapping between its output and $\mathcal{BN}$, every feasible path in $\mathcal{BN}$ is a VF-path.
}
\end{proof}
\begin{lemma}
Every feasible path from $j$ to a node $i$ in the $\mathcal{BN}$ graph, is an eligible VF-path (from $i$ to $j$).
\end{lemma}
\begin{proof}
\pavlos{TO PROVE (use again the fact that every incoming edge to a node is of the same type c2p / p2p / p2c, and prove by contradiction)}\\
\vkotronis{According to the previous lemma, all feasible paths in $\mathcal{BN}$ are VF-paths. Following the eligible VF-path formation process of Algorithm~\ref{alg:all-vf-paths}, whose output is then fed to the $\mathcal{BN}$ formation, guarantees that for every node in $\mathcal{N}\setminus\{j\}$: (i) all incoming edges to the node are of the same type, and (ii) all outgoing edges from the node are of the same type, and (iii) these are the most preferred (according to VF) types to reach $j$. Assume that there is a feasible path from $j$ to $i$ that is VF (according to the previous lemma), but not eligible. This means that there is a ``better'', eligible path between these nodes, hence at least one of the nodes on the path should be able to route traffic using a more preferred neighbor. However, according to the reasoning of the previous 3 points (i), (ii) and (iii), this is not possible (proof by contradiction).
Therefore, every feasible path from $j$ to $i$ is an eligible VF-path.}\\
%\vkotronis{Following a sequence of directed edges between $i$ and $j$ (in the reverse direction) is equivalent to following an eligible VF-path from $i$ to $j$; each edge sequence corresponds 1-to-1 to an eligible VF-path, and thus $\mathcal{BN}$ contains \textit{only} eligible-VF paths.}
\end{proof}
The above Lemmas tell us that the VF-BN is an equivalent representation of all the eligible VF-paths.

Fig.~\ref{fig:example-BN} shows an example of the VF-BN graph that contains the eligible VF-paths to node $j$. 


\begin{figure}
\centering
\includegraphics[width=0.8\linewidth]{./figures/example_BN.eps}
\caption{Example VF-BN. \pavlos{TODO: add also a link from a to f.} \pavlos{TODO: add also a node $h$ between d and g.}}
\label{fig:example-BN}
\end{figure}

\begin{algorithm}[t]
\caption{Build the VF-BN.}
\label{alg:build-vf-bn}
\begin{algorithmic}[1]
% input:
\Statex {\textbf{Input:} network graph $\mathcal{G}(\mathcal{N},\mathcal{E})$; all eligible VF-paths $\mathcal{P}$.}
% algorithm
\State $\mathcal{BN}(\mathcal{N}_{BN}, \mathcal{E}_{BN})\leftarrow \emptyset$ \Comment initialization of the BN graph
\State $\mathcal{N}_{BN}\leftarrow \mathcal{N}$
\For {$path\in \mathcal{P}$}
	\For {$e_{i,j}\in path$}
    	\State $\mathcal{E}_{BN}\leftarrow \mathcal{E}_{BN}~\cup~\{(j, i)\}$
    \EndFor
\EndFor
\State \Return $\mathcal{BN}$
\end{algorithmic}
\end{algorithm}


\subsection{Step 4 - BN-based best path prediction}
Our goal is to find, for all nodes $i\in\mathcal{N}$, through which peering point of $j$ they route traffic to it \vkotronis{I think this is a good time to introduce why we want to do this; will this be in the intro? E.g., ``Prediction of Anycast Catchment'', ``Hijack Pollution Estimation'', etc.?}. For instance, in the example of Fig.~\ref{fig:example-BN}, we want to find for the nodes $\{c,d,e,f,g\}$ whether they route traffic to $j$ through node $a$ or node $b$. 

To visualize this, we can assign to nodes $a$ and $b$ different ``colors''; our goal is to color the remaining nodes in the VF-BN. If a node $i$ has a best path to $j$ through node $a$ \vkotronis{Maybe here we can say ``If all preferred VF-paths of node $i$ pass though node $a$? We do not know the best path.''}, then it has the same color as $a$, and we denote \vkotronis{Is this denotation normally used in similar contexts?} it as
\begin{equation*}
i\rhd a
\end{equation*}

In the example of Fig.~\ref{fig:example-BN}, it is easy to see that $c$ has only one VF-path to $j$, through $a$, and thus $c\rhd a$. Similarly, $e\rhd b$. However, for node $d$ there are two possible VF-paths, one through $a$ and one through $b$. Hence, without further knowledge on the routing policies/preferences \pavlos{to better define what I mean here. I mean if we do not know local neighbor preferences and/or if node prefers shorter paths for all neighbors of same type.} \vkotronis{yes this is clear} of $d$, we cannot assign to it a certain color. On the contrary, although node $f$ has two possible paths to $j$, both of them are through node $a$. Hence, we can color node $f$ as $f\rhd a$.

\myitem{Observation 1: \vkotronis{The naive coloring process} might not be able to color all nodes in the VF-BN graph, if the routing policies are not known for every node.}

To find which nodes can be colored, under unknown routing policies/preferences, we apply Algorithm~\ref{alg:coloring-vf-bn}. In sum, Algorithm~\ref{alg:coloring-vf-bn} starts from the peering points of the destination node and colors them with different colors (\textit{lines 5--8}). Then, sequentially visits nodes that are closer to the destination node, by following a topological ordering of the VF-BN nodes (\textit{line 9}), which is defined as
\begin{definition}[Topological sort]\label{def:topological-sort}
A topological sort/ordering $\mathcal{T}$ of a directed graph $\mathcal{G}(\mathcal{N},\mathcal{E})$ is a linear ordering of its nodes $\mathcal{N}$ such that for every directed edge $e_{ij}\in\mathcal{E}$ from node $i\in\mathcal{N}$ to node $j\in\mathcal{N}$, $i$ comes before $j$ in the sort/ordering $\mathcal{T}$\footnote{\vkotronis{Note that the coloring of nodes on the ``same'' level (i.e., at the same distance from the root of the DAG) does not affect the coloring of each other, therefore any --even random-- order is acceptable.}}.
\end{definition}
%\vkotronis{How does this definition handle node ``on the same level''? Is the order random in that case?}\pavlos{We don't mind for the order of nodes "on the same level", since they do not affect the coloring of each other. I.e., any (random) order for same-level-nodes is fine} \vkotronis{OK then I will mention it as a footnote}

Each visited node is colored if all its predecessor nodes have the same color (\textit{lines 10--23}). If some of is predecessors has no certain color (\textit{lines 15--17}) or predecessors have more than one colors (condition in \textit{line 20} is not satisfied because $|CP|>1$), then the color of the node is left undefined.




\begin{algorithm}[t]
\caption{Coloring of the VF-BN.}
\label{alg:coloring-vf-bn}
\begin{algorithmic}[1]
% input:
\Statex {\textbf{Input:} VF-BN graph $\mathcal{BN}(\mathcal{N}_{BN}, \mathcal{E}_{BN})$; destination node $j$.}
% algorithm
\State $CD\leftarrow \emptyset$ \Comment The coloring dictionary of the VF-BN
\For {$i\in\mathcal{N}_{BN}$}
	\State $CD[i]\leftarrow \emptyset$
\EndFor
\State $PP_{j}\leftarrow$\textproc{get\_descendants}($j,\mathcal{E}_{BN}$)
\For {$i\in PP_{j}$}
	\State $CD[i]\leftarrow i$
\EndFor
\State $\mathcal{T}\leftarrow$\textproc{topological\_sort($\mathcal{BN}$)}
\For {$i\in \mathcal{T}\backslash\{j\cup PP_{j}\}$}
  	\State $CP\leftarrow \emptyset$
	\For {$j\in$ \textproc{get\_predecessors}($i,\mathcal{E}_{BN}$)}
    	\If {$CD[j]\neq \emptyset$}
    		\State $CP\leftarrow CP\cup CD[j]$
        \Else
        	\State $CP\leftarrow\emptyset$
        	\State \Break
        \EndIf
    \EndFor
    \If{$|CP|=1$}
    	\State $CD[i]\leftarrow CP$
    \EndIf
\EndFor
\State \Return $CD$
\end{algorithmic}
\end{algorithm}




\myitem{Observation 2: Weak path ordering can increase the coloring coverage of the strict path ordering.} \pavlos{We could also express this as lemma/corollary/etc as well; it can be easily proved , because the weak-VF-BN has less edges, and the uncertainty decreases (or, does not increases) when an edge is removed.} \vkotronis{I think the latter statement is a bit weaker; I understand the concept but we need to support it more formally.}

In the above process, we colored the nodes for which we could infer with certainty the preferred paths, based on the node relationships, \ie we applied a \textit{strict ordering} of paths. Relaxing this condition \vkotronis{do we really relax this condition? I think we preserve the condition and we apply and extra filter to keep only the weakly preferred paths among the strictly preferred ones.}, and assuming that nodes always prefer the shortest paths (received from neighbors of the same type), we can apply an \vkotronis{additional} \textit{weak ordering} of the paths, to infer the color for some extra nodes. 

To take into account weak path ordering, we transform the VF-BN according to Algorithm~\ref{alg:transform-vf-bn-weak}. For each node we remove the incoming edges that correspond to longer paths to the destination $j$. Since all incoming links to a node are from neighbors of the same type, under weak ordering only the shortest link(s) will be preferred. Hence, if a predecessor has a path longer than any of the other predecessors, it will never be preferred, and thus this link can be \vkotronis{safely} removed from the VF-BN.

\begin{algorithm}[t]
\caption{Transformation of the VF-BN with weak path ordering.}
\label{alg:transform-vf-bn-weak}
\begin{algorithmic}[1]
% input:
\Statex {\textbf{Input:} VF-BN graph $\mathcal{BN}(\mathcal{N}_{BN}, \mathcal{E}_{BN})$; destination node $j$.}
% algorithm
\State $L\leftarrow \emptyset$ \Comment The min path length dictionary of the VF-BN
% \For {$i\in\mathcal{N}_{BN}$}
% 	\State $L[i]\leftarrow \infty$
% \EndFor
\State $L[j]\leftarrow 0$; $L[i]\leftarrow \infty,~\forall i\in\mathcal{N}_{BN}\backslash\{j\}$ 
\State $\mathcal{T}\leftarrow$\textproc{topological\_sort($\mathcal{BN}$)}
\For {$i\in \mathcal{T}\backslash\{j\}$}
	\For {$k\in$ \textproc{get\_predecessors}($i,\mathcal{E}_{BN}$)}
    	\State $L[i] \leftarrow \min\{L[i], L[k]+1\}$
    \EndFor
    \State $\mathcal{E}_{BN} \leftarrow \mathcal{E}_{BN} - \{e_{ki}\in\mathcal{E}_{BN}: L[k]+1 > L[i]\}$
%     \For {$k\in$ \textproc{get\_predecessors}($i,\mathcal{E}_{BN}$)}
%     	\If {$min\_length < L[k]+1$}
%     		\State $\mathcal{E}_{BN} \leftarrow \mathcal{E}_{BN} - \{e_{ki}\}$
%         \EndIf
%     \EndFor
\EndFor
\State \Return $\mathcal{BN}(\mathcal{N}_{BN}, \mathcal{E}_{BN})$
\end{algorithmic}
\end{algorithm}

\vkotronis{@pavlos: could you explain this equation in-text?}


\myitem{Coloring of nodes can be extended to probabilistic coloring of nodes, by assuming (or, having) further knowledge on local neighbor preferences.}
\vkotronis{Will we introduce probabilistic coloring here?}\pavlos{YES, we will introduce. But, the probabilistic coloring could be formally introduced using terminology of BN and conditional probabilities, (and maximum likelihood prediction), etc.; need to read a bit more on BN, to see how to write it in a formal way.}
%DEPRECATED
%\vkotronis{``We use a probabilistic bayesian classifier (based on the eligible/preferred VF dependencies between the nodes), which for any node $i$ in the graph, returns one of $PP$ possible states, where $PP$ is the set of peering points via which node $j$ is connected to the rest of the graph.''}

\begin{equation}
i\rhd \arg\max_{i\in PP_{j}} P\{a\rhd i | CD[k]:~\forall k\in \mathcal{N}_{BN}, e_{ki}\in\mathcal{E}\}
\end{equation}



\subsection{Coloring with measurements}
The initial coloring of the VF-BN can be augmented with measurements, \eg from BGP monitoring services (passive measurements), or pings/traceroutes (active measurements).

A measurement can determine the color of 
\begin{itemize}
\item the measured node
\item all the nodes in the measured path \vkotronis{(towards the intended destination)} for the measured node (in case of path measurements, such as BGP path or traceroute; this is not possible with ping measurements)
\item the nodes that are related to the measured node (children and parents), depending on the (a) VF-BN structure and (b) color of \vkotronis{already} measured nodes.
\end{itemize}
We design Algorithm~\ref{alg:coloring-from-measurements} for performing graph coloring with measurements. \vkotronis{@pavlos: we need to describe the algorithm as the rest in-text, but I do not understand all steps efficiently. Could you explain on high-level or some interesting lines?}

\begin{algorithm}[t]
\caption{Coloring from measurements.}
\label{alg:coloring-from-measurements}
\begin{small}
\begin{algorithmic}[1]
% input:
\Statex {\textbf{Input:} VF-BN graph $\mathcal{BN}(\mathcal{N}_{BN}, \mathcal{E}_{BN})$; destination node $j$; measurements $\mathcal{M}$; coloring probabilities $\pi_{i}(c)~\forall i\in\mathcal{N}_{BN},c\in\mathcal{PP}_{j}$.}
% algorithm
\Statex \underline{Initialization}
\State $\mathcal{CD}\leftarrow \emptyset$ \Comment dictionary of colors from measurements
\For {$i\in\mathcal{M}$}
	\State $CD[i]\leftarrow$\textproc{get\_color\_from\_measurement($\mathcal{M}$)}
    \If {path\_measurements}
    	\For {$k\in path_{ij}$}
        	\State $CD[k]\leftarrow CD[i]$
        \EndFor
    \EndIf
\EndFor
\State $\mathcal{L}\leftarrow \{i\in\mathcal{N}_{BN}:CD[i]\neq \emptyset\}$ \Comment list of nodes to color
\Statex \underline{Recursive coloring}
\While {$\mathcal{L}\neq \emptyset$}
	\State $i\leftarrow$ \textproc{get\_first\_node}($\mathcal{L}$)
    \State $C_{i}\leftarrow \{c\in\mathcal{PP}_{j}: \pi_{i}(c)>0\}$
    \If {$CD[i]\notin C_{i}$}
    	\State \textproc{fix\_graph()}
    \Else
    	\If {$|C_{i}|=1$}
        	\State \textbf{continue}
        \Else \Comment \ie $|C_{i}|>1$
        	\State $\textproc{color\_node}(i,CD[i])$
            \State $PI_{i}\leftarrow \{k\in\textproc{get\_parents}(i):\pi_{k}(CD[i])>0\}$ 
            \If {$|PI_{i}|=1$}
            	\State $\mathcal{L}\leftarrow \mathcal{L}\cup \{PI_{i}\}$
                \State $CD[PI_{i}] = CD[i]$
            \Else \Comment \ie $|PI_{i}|>1$
            	\State \textbf{continue}
            \EndIf
        \EndIf
    \EndIf
\State $\mathcal{L}\leftarrow\mathcal{L}\backslash\{i\}$
\EndWhile

\Statex 
\Function{color\_node}{$i,c$}
\State $\pi_{i}(c)\leftarrow 1$; $\pi_{i}(d)\leftarrow 0,~~\forall d\neq c$
\State $CI_{i}\leftarrow \textproc{get\_children}(i)\backslash \mathcal{L}$
\For {$k\in CI_{i}$}
	\If {$\{\ell\in\textproc{get\_parents}(k): \pi_{\ell}(c)<1\}=\emptyset$}
    	\State $\mathcal{L}\leftarrow \mathcal{L}\cup \{k\}$
        \State $CD[k] = c$
    \EndIf
\EndFor
\EndFunction
\end{algorithmic}
\end{small}
\end{algorithm}



==> PathPrepending_backup.tex <==
\myitem{Example application: TE through path prepending.} \pavlos{TBD if/where to add this}\vkotronis{@pavlos: I moved it in the form of a comment (and shortened it a bit) to Section~\ref{sec:disc-app}. Please check and if you agree simply comment out the current content here (do not delete)}%
\blue{
It is common for network operators to use path prepending for traffic engineering (TE) purposes. For example, a $n_{dst}$ may announce the same prefix differently to its two upstream providers / \ppoints $m1$ and $m2$:
\begin{align*}
    \text{announcement to m1} \rightarrow & [n_{dst}]\\
    \text{announcement to m2} \rightarrow & [n_{dst}, n_{dst}, ..., n_{dst}]
\end{align*}
aiming to increase the traffic through $m1$ (paths through $m2$ will be longer and de-preferred by some nodes). The longer the prepending, the less the catchment of $m2$. However, \textit{how many times does $n_{dst}$ need to prepend its ASN to achieve the desired balance between the catchment of its \ppoints}? Algorithm~\ref{alg:transform-vf-bn-weak} allows to answer the above question efficiently (with 
low computation complexity). 
}

\blue{
First, note that path prepending can be captured in the \Rgraph by adding a number of ``virtual'' nodes (equal to %those in prepending
the number of extra prepended ASNs) between $n_{dst}$ and $m2$. Apart from this change, the \Rgraph remains the same, since the eligible paths are independent of the path lengths. Hence, we can create an \Rgraph for each path prepending option, simply by duplicating the original \Rgraph and adding the corresponding number of virtual nodes. Then, for each \Rgraph we can apply Algorithms~\ref{alg:transform-vf-bn-weak} and~\ref{alg:coloring-vf-graph} to infer the catchment of the \ppoints. The complexity of this task is much lower than performing BGP simulations for each prepending case (which would be required by existing approaches). For instance, to examine $K$ path prepending scenarios would require $K$ BGP simulations of complexity $O(|\mathcal{N}|\cdot |\mathcal{E}|)$, whereas we need to run \textit{only once} Algorithm~\ref{alg:build-vf-graph} of complexity $O(|\mathcal{N}|\cdot |\mathcal{E}|)$ and then run $K-1$ times Algorithms~\ref{alg:transform-vf-bn-weak} and~\ref{alg:coloring-vf-graph} whose complexity is $O(|\mathcal{N}|+ |\mathcal{E}|)$ (which is $\ll O(|\mathcal{N}|\cdot |\mathcal{E}|)$ in all practical scenarios).
}

==> Preliminaries.tex <==
\subsection{Definitions}
\begin{itemize}
\item $\mathcal{AS}$: the set of ASes in the Internet 
\item $X$: the the network of interest; $X\in\mathcal{AS}$
\item $\mathcal{N}$: the peering points of $X$
\item $pfx_{i}$: a prefix advertised by $i$; $i\in\mathcal{AS}$.
\item $path_{ij}$: the (best) AS path from $i$ to $j$; $i,j\in\mathcal{AS}$. A path is denoted as $path_{ij} = [i, ASx, ASy, ..., ASz, j]$.
\end{itemize}


\subsection{Information Sources}
In our methodology we use information about the Internet routing (layer-3). Such information can be provided from the following sources.
\begin{itemize}
\item \textbf{BGP data} sources, such as (i) route collectors (BGPStream, RIPE RIS) and (ii) looking glass (LG) servers, can provide information about the BGP paths (or, equivalently, AS paths).
\item \textbf{Traceroute measurements} provide information about IP paths. Mapping IP-to-AS information gives AS paths, which can be used similarly to BGP paths. RIPE Atlas can be used to conduct and/or collect traceroute measurements.
\pavlos{Traceroutes over RIPE Atlas:
\begin{itemize}
\item $\sim$10k probes
\item in $\sim$2.7k ASes
\item default measurements: $\sim$100 per probe per day
\item user-defined measurements: $\sim$170k credits for measurements from \textit{all ASes with a probe} to a prefix (\ie $\sim$2.7k measurements)
\end{itemize}
}
\item \textbf{AS-graph} information (\eg CAIDA's dataset) can be combined with the \textbf{GR-model} to provide information / infer routing on the Internet.
\end{itemize}

The characteristics of the information sources, with respect to (i) how easy is their collection or use, (ii) the correctness (or, accuracy) of the provided information, and (iii) the completeness of the information, are given in Table~\ref{table:information-sources}.
\begin{table}[h]
\centering
\caption{Characteristics of information sources.}
\label{table:information-sources}
\begin{tabular}{l|ccc}
{}						& {BGP data}	& {Traceroutes}	& {GR-model}\\
\hline
{Easy to collect / use}	& {\cmark}		& {\xmark}		& {\cmark}\\
{Correctness}			& {\cmark}		& {\cmark (?)}	& {\xmark}\\
{Coverage}				& {\xmark}		& {\cmark (?)}	& {\cmark}\\
\end{tabular}
\end{table}

\todo{Quantify the characteristics in Table~\ref{table:information-sources}. Specifically,
\begin{itemize}
\item Coverage of BGP data: How many ASes have monitors (route collectors) or LGs? \vkotronis{We have this info from the ARTEMIS paper right? And we probably read info from VG's Periscope.}
\item Correctness of traceroutes: What is the error in IP paths to AS paths? \vkotronis{That is an extremely hard question, are you sure we can address this in the paper?}
\item Coverage of traceroutes: How many ASes have RIPE Atlas probes? \vkotronis{we can get this info from Petros quickly I think.}
\item Correctness of GR-model: How many paths or first-hop-neighbors (or other metric?) are wrong in GR sims?\\ \vkotronis{Since we do not have ground truth on this, but only Phillipa's paper which makes inferences based on a limited survey, I am not sure how to respond to this.} 
Also, write why the GR model is not accurate, namely (i) for definite decisions on path selections, we need to know local preferences, which we do not know, and (ii) but even relationships are only 70\% accurate according to [ref].  
\end{itemize}
}
\todo{From the CAIDA graph we can find the ASes that have a single upstream. If an AS has a single upstream we can group it with its upstream. We are interested in the \textit{groups of ASes} (~10k) rather than all the ASes (~65k). Hence:
\begin{itemize}
\item Build list of group of ASes from CAIDA graph
\item Validate this list (to what extend it holds) against real data from (i) BGP sources and/or (ii) traceroutes. For instance, check if a different upstream appears in any of the BGPpaths.)
\vkotronis{This is not a validation, since it is still heavily biased by the presence and location of the control-plane monitors. It is only an indication; and already BGPStream takes advantage of almost all potential collectors in the world. So I do not get how we can validate based on BGP sources. Regarding traceroutes: note that data-plane traffic can be inconsistent with control-plane state (static routes, best path vs multipath, etc.). So it does not make sense from my point of view to validate the control-plane using the data plane. Since this is a longer and critical discussion, let's make it in person.}
\end{itemize}
}


\subsection{Validation of the Key Idea}
\underline{Question:} \textit{Is it possible to use information about the existing paths to predict paths after routing changes?}

Our approach towards answering the above question is the following. Let us assume that ``now'' $X$ is not connected with any of the peering points $\mathcal{N}$. The information we have ``now'' is only the paths $path_{ij}$, where $i\in\mathcal{AS}$ and $j\in\mathbb{N}$, for the prefixes $pfx_{j}$. Information about the paths $path_{iX}$ for a prefix $pfx_{X}$, will be available only after $X$ establishes connections to all peering points $\mathcal{N}$. Hence, we need to know if it is possible to infer from $path_{ij}$ the $path_{iX}$.

\pavlos{Note: this is not always the case; only when $X$ is a customer of all $N$ points.}

\vkotronis{Could you elaborate on this statement? Why only in this case? When for example it is a peer it does not mean that it will be preferred, is this the intuition?}

\begin{conjecture}\label{conjecture:anycast-path-in-best-paths}
The path from a network $i$ to $X$ (for $pfx_{X}$) will be equal to the path from $i$ to a peering point $j$ of $X$  (for $pfx_{j}$) appended by $X$, \ie 
\begin{equation}\label{eq:anycast-path-in-best-paths}
path_{iX} \in \{[path_{ij}, X]: j\in\mathcal{N}\}
\end{equation}
\end{conjecture}

We test Conjecture~\ref{conjecture:anycast-path-in-best-paths} through simulations. We present the results in Table~\ref{table:percentage-paths-anycast} and Fig.~\ref{fig:comparison-best-anycast-paths-boxplot}.\todo{\pavlos{} (Re-)caclulate these results for the ``groups of ASes'', and not all ASes.} On average (over different cases of $X$ and $\mathcal{N}$), for more than $95\%$ of the networks $i\in\mathcal{AS}$ the Conjecture~\ref{conjecture:anycast-path-in-best-paths} \vkotronis{holds}. For the remaining networks $i$, we investigate why the conjecture does not hold.\pavlos{What are the path lengths for these cases?} In $75\%-80\%$ of these cases, networks have a different path, because they select a path from a different provider, and in $20\%-25\%$ of the cases the networks $i$ select the same next hop, but the path changes in a later hop (closer to $X$). \pavlos{Note that we have simulated only cases that $X$ is a customer to all $j\in\mathcal{N}$, \ie anycast cases. Maybe think better, if the simulation setup needs to be modified.}

\begin{table}
\centering
\caption{Percentage (\%) of cases that $path_{iX} \in \{[path_{ij}, X]: j\in\mathcal{N}\}$.}
\label{table:percentage-paths-anycast}
\begin{tabular}{c|cccccccc}
{\# anycasters}&{3}&{4}&{5}&{6}&{7}&{8}&{9}&{10}\\
\hline
mean value& {95.6}&{95.8}&{96.3}&{96.5}&{96.8}&{97}&{97.2}&{97.2}\\
median values&{98.3}&{98}&{97.6}&{97.8}&{98}&{98.1}&{98.2}&{98.2}\\
\end{tabular}
\end{table}

\begin{figure}
\centering
\subfigure[anycast]{\includegraphics[width=0.45\linewidth]{./figures/fig_comparison_best_anycast_paths_boxplots.eps}\label{fig:comparison-best-anycast-paths-boxplot}}
\subfigure[anycast]{\includegraphics[width=0.45\linewidth]{./figures/fig_comparison_best_anycast_paths_percentage_next_hop_type_only_different_paths.eps}\label{fig:comparison-paths-next-hop-type-anycast}}
\caption{(a) Boxplots for the percentage of same best paths ($path_{ij}$) and paths to anycasters ($path_{iX}$). \pavlos{Maybe the CDF will better show the behavior; however, many CDFs on the same plot might be difficult to read.} (b) Mean percentages of the different tuples of next hop types for the best paths and anycasting path the anycasting, when $path_{iX} \in \{[path_{ij}, X]: j\in\mathcal{N}\}$ (which is a small fraction, $<5\%$, of the total cases; see results in (a)). The notation in the legend denotes the type of the next hop in the best path (first letter) and common path (second letter); \textit{c} is for customer, \textit{p} for peer, \textit{P} for provider, and \textit{same} if the next hop is the same AS (but the entire CP is not the same with the BP).}
\label{fig:comparison-paths-boxplots}
\end{figure}


\todo{Depict an example scenario where Conjecture~\ref{conjecture:anycast-path-in-best-paths} does not hold.}

\todo{Test the validity of Conjecture~\ref{conjecture:anycast-path-in-best-paths} with real data as well: BGP and/or traceroutes. For example
\begin{itemize}
\item Consider an AS $X$ and a prefix $pfx_{X}$, and all its neighbors $\mathcal{N}$ (select only those to which $X$ advertises $pfx_{X}$). Check paths of all available vantage points $i\in\mathcal{AS}$ to the prefixes $pfx_{X}$ and $pfx_{j}$, $j\in\mathcal{N}$.
\item AND/OR, consider a MOAS pfx and let the MOAS ASes be the set $\mathcal{N}$. Compare paths of all available vantage points $i\in\mathcal{AS}$ to the MOAS prefix and to the prefixes $pfx_{j}$, $j\in\mathcal{N}$.
\end{itemize}
}


==> Results_backup.tex <==
In this section, we apply the model of Section~\ref{XXX}, the basic route inference methodology of Section~\ref{YYY}, and its extensions related to measurement-enhanced inference (see Section~\ref{WWW}) and preference of shorter paths (see Section~\ref{ZZZ}) in order to infer the routes (colors) of the nodes contained in the AS-relationship graph, towards different sets of anycasters.

\subsection{Experimental Setup \& Datasets}

\myitem{The Graph.} We first build the AS-level topology graph using CAIDA's AS-relationship dataset~\cite{}, which is collected based on the methodology of ~\cite{} and enriched\footnote{Besides using CAIDA's AS-relationship graph as-is, we also repeated all our experiments using extra peering links from PeringDB~\cite{}, by considering p2p links between IXP members adopting an ``Open Policy'' peering with all other members of the same IXP. However, this addition did not change our results; therefore, to eliminate any added ambiguity due to potential inaccuracies in PeeringDB, we present only results based on the initial graph generated via CAIDA's dataset.} with extra peering links~\cite{}. The dataset contains a list of AS pairs with a peering link, which is annotated based on a p2p pr p2c relationship.

\myitem{Monitors.} In order to achieve inference enhancement by exploiting passive or active measurements from ASes hosting route monitors, we consider the following sets of monitors\footnote{Note that we do ``simulated'' measurements according to the capabilities that each class of monitors (ASes) offers: e.g., RIPE Atlas probes can either ping, uncovering the destination-facing peering point, or traceroute, uncovering the entire path to the destination}:

\begin{itemize}

\item \textbf{RouteViews.} RouteViews~\cite{} provides control-plane information (BGP RIBs and updates) collected from 19 route collectors that are connected to more than 400 ASes worldwide. All data can be accessed using tools from
BGPStream~\cite{}.

\item \textbf{RIPE RIS.} RIPE’s Routing Information System (RIS)~\cite{} has more than 20 route collectors (RCs) distributed worldwide, collecting BGP RIBs and updates from around 300 peering ASes. 
Data from all RCs can be accessed (with a delay of a
few minutes) through RIPEstat~\cite{} or the tools of CAIDA’s
BGPStream~\cite{} framework.

\item \textbf{RIPE Atlas.} RIPE Atlas~\cite{} a well-established global Internet measurement platform with more than 25,000 probes, i.e., measurement devices hosted in homes, IXPs, co-location facilities, etc. Using the RIPE Atlas API~\cite{}, we fetch all ASes hosting RIPE Atlas monitors which can execute either pings or traceroutes towards certain destination prefixes. Since in our results we consider only IPv4-anycasted prefixes, we account for ASes hosting IPv4 probes; this yields $\sim$3.5K ASes.

\item \textbf{Looking Glasses.} Using the Periscope platform~\cite{}, we list 883 Looking Glass servers which can be used to examine the BGP RIBs of the ASes hosting them; in some cases they can even perform limited active measurements such as pings and traceroutes.

\item \textbf{IXP Route Servers.} Using data from PeeringDB~\cite{} we identify 560 IXPs around the globe with an aggregate peering base (i.e., set of IXP members) reaching 6.5K members. Assuming that each of them hosts a Route Server (a very common practice to scale up the BGP peering mesh within an IXP), we use the BGP RIBs that these vantage points would observe, as exported by the respective IXP members.

\end{itemize}

\myitem{BGP Simulator.} We build a custom BGP simulator taking as input the AS-relationship graph and operating on valley-free conventions, to simulate BGP and implement the ``RUNBGP'' function of Algorithm~\ref{alg:build-vf-graph}. The simulator operates based on the following simple --distributed-- logic. When an AS learns a new route for a prefix (or, announces a new prefix), it updates its routing table and, if required, sends BGP updates to its neighbors. The update and export processes are determined by its routing policies.

\myitem{Prefix-to-AS.} To find out which are the truly anycasted prefixes appearing in the Internet, we employ CAIDA's \texttt{pfx2as} dataset~\cite{} containing mappings of IP prefixes to the ASes that advertise them. Anycasted prefixes and their respective sets of anycasters are explicitly marked.

\myitem{BGPStream Datasets.} As described previously, BGPStream~\cite{} can be used to access the BGP RIBs of all RIPE RIS and RouteViews route collectors at different points in time. To validate our findings, we download these RIBs using the same date as the one when the CAIDA dataset was generated. Using these RIBs we can check directly how the contained ASes route traffic to different anycasted prefixes, and thus different sets of anycasters. Note that we consider only prefixes for which: (i) routes are towards anycasters yielded from CAIDA's \texttt{pfx2as} dataset, and (ii) more than 50\% of the total RouteViews-RIPE RIS monitors have seen at least one path towards the anycasters, and (iii) anycasters appear only once per observed path, and (iv) the measured catchment of any anycaster for a specific anycasted prefix is less than 90\%. In total, we have information for \red{X} anycasted prefixes.

\subsection{Coverage}

We first perform simulations to estimate the percentages of colored nodes with respect to the entire AS population, for random prefixes and sets of anycasters of different size (2,4,8 and 16 anycasters). Using the AS-relationship graph and our BGP simulator, we first build the VF $\mathcal{G_{BN}}$ graph using Algorithm~\ref{}. Then, assuming no measurement-based enhancements from monitors (``NO\_MON''), we perform inference on the yielded graph using Algorithm~\ref{}. We further enhance this inference using Algorithm~\ref{}, by assuming different sets of monitors, i.e., RouteViews and RIPE RIS (``RV\_RIS''), IXP Route Servers (``IXP\_RS''), RIPE Atlas ping probes (``RA\_PING''), RIPE Atlas traceroute probes (``RA\_TRACE''), Looking Glass servers (``LG'') and the union of all aforementioned monitors (``ALL''). Finally, we consider both preferences based solely on the strict route inequality related to the class of the neighbor of the AS (e.g., customer, peer, provider --``STRICT''), as well as a combination of policy-based and shortest path preference assuming a weak, path length-based, inequality between preferred neighbors of the same class (using Algorithm~\ref{} --``WEAK'').
The relevant results are presented in Fig.~\ref{fig:color_cov_perc} for the strict (Fig.~\ref{fig:color_cov_perc_strict}) and weak (Fig.~\ref{fig:color_cov_perc_weak}) case.
We observe that: \todo{which monitors are better, which route preference is better, etc...}

\subsection{Accuracy}

After calculating the node colors using simulations in the previous step, we focus on the no-measurement case to compare our inferences/predictions ($sim$) against real-world measured datasets (BGP RIBs) from BGPStream (ground truth $gt$). The colors of the nodes involved in the $gt$ paths can be directly measured \footnote{Note that there are cases where a certain node (AS) routes to different anycasters due to its distributed topology and different policies across its network. We leave these cases out of the comparison as inconsistent routes.}. We calculate the following:

\begin{itemize}
\item $common\_colored = \{n \in \mathcal{N}_{sim}\bigcap{}\mathcal{N}_{gt}, \exists! m \in \mathcal{M}, s.t. n \rhd_{sim} m \wedge \exists! m \in \mathcal{M}, s.t. n \rhd_{gt} m\}$
\item $same\_colored = \{n \in \mathcal{N}_{sim}\bigcap{}\mathcal{N}_{gt}, \exists! m \in \mathcal{M}, s.t. n \rhd_{sim} m \wedge n \rhd_{gt} m\}$
\item $diff\_colored = \{n \in \mathcal{N}_{sim}\bigcap{}\mathcal{N}_{gt}, \exists! m_1 \in \mathcal{M}, s.t. n \rhd_{sim} m_1 \wedge \exists! m_2 \in \mathcal{M}, s.t. n \rhd_{gt} m_2 \wedge m_1 != m_2\}$
\item $same\_color\_perc = 100.0*\frac{|same\_colored|}{|common\_colored|}$
\item $diff\_color\_perc = 100.0*\frac{|diff\_colored|}{|common\_colored|}$
\item $gt\_coverage = 100.0*\frac{|common\_colored|}{|n \in \mathcal{N}_{gt}, \exists! m \in \mathcal{M}, s.t. n \rhd_{gt} m|}$
\end{itemize}

\vkotronis{REMINDER: need to update the results of the gt vs sim comparison when all data are available! This is only for 84 truly anycasted prefixes.}

\todo{we observe that...}

%\pavlos{Idea: what about if we remove all stubs (independently of the number of providers they have) and consider only the remaining nodes in the graph. We have no information about how stubs with more than one providers route their traffic (maybe one of them is backup), so when considering them we (i) require more measurements (in theory and practice), and (ii) get lower accuracy in practice.} \vkotronis{I am not sure, we diminish the contribution a lot then since multi-homed stubs are a significant percentage that we should be able to color. Otherwise we focus essentially only on transit ISPs which is not the whole Internet, but a --ok, well-connected-- portion of it.}

\begin{figure}
\centering
\subfigure[strict preference]{\includegraphics[width=0.45\linewidth]{./figures/color_cov_strict.eps}\label{fig:color_cov_perc_strict}}
\subfigure[weak preference]{\includegraphics[width=0.45\linewidth]{./figures/color_cov_weak.eps}\label{fig:color_cov_perc_weak}}
\caption{Distribution of the percentage of nodes with certain color (y-axis) under different number of anycasters (x-axis), for cases (i) without measurements, and with measurements from (ii) IXP Route Servers, (iii) BGP route collectors, (iv) LG servers, (v) RIPE Atlas probes, and (vi) all available VPs, for the (a) strict and (b) weak DAG route preference. Each boxplot corresponds to a 1000 simulation runs, with randomly varying $q_{ij}$s.}
\label{fig:color_cov_perc}
\end{figure}

\begin{figure}
\centering
\subfigure[strict preference]{\includegraphics[width=0.45\linewidth]{./figures/compare_cdf_strict_0_0.eps}\label{fig:compare_cdf_strict_0_0}}
\subfigure[weak preference]{\includegraphics[width=0.45\linewidth]{./figures/compare_cdf_weak_0_0.eps}\label{fig:compare_cdf_weak_0_0}}
\caption{Percentages of nodes with same or different color belonging to both the simulated (inferred) and ground truth datasets, as well as the coverage of the ground truth dataset achieved by the simulated inference methodology for the (a) strict and (b) weak DAG route preference.}
\label{fig:compare_cdf_0_0}
\end{figure}

\begin{figure}
\centering
\subfigure[\vkotronis{10\% ground truth links}]{\includegraphics[width=0.45\linewidth]{./figures/compare_cdf_weak_0_1.eps}\label{fig:compare_cdf_weak_0_1}}
\subfigure[\vkotronis{20\% ground truth links}]{\includegraphics[width=0.45\linewidth]{./figures/compare_cdf_weak_0_2.eps}\label{fig:compare_cdf_weak_0_2}}
\caption{\vkotronis{Percentages of nodes with same or different color belonging to both the simulated (inferred) and ground truth datasets, as well as the coverage of the ground truth dataset achieved by the simulated inference methodology for the weak DAG route preference, after considering (a) 10\% and (b) 20\% of the preferred ground truth links closest to the anycaster(s).}}
\label{fig:compare_cdf_0_0}
\end{figure}

% \pavlos{I added some placeholders for the figures in this section.}

% \begin{figure}
% \centering
% \subfigure[\pavlos{min path length}]{\includegraphics[width=0.45\linewidth]{./figures/empty.eps}\label{fig:}}
% \subfigure[\pavlos{\#leaf nodes}]{\includegraphics[width=0.45\linewidth]{./figures/empty.eps}\label{fig:}}
% \caption{\pavlos{Properties of the DAG (VF-BN). (a) Distribution of the min path length (from the root) over all nodes (y-axis) for different number of anycasters (x-axis). (b) Distribution of the number of leaf nodes (y-axis) for different number of anycasters (x-axis). Results both for strict and weak DAG are presented.} }
% \label{fig:}
% \end{figure}

% \begin{figure}
% \centering
% \subfigure[]{\includegraphics[width=0.45\linewidth]{./figures/empty.eps}\label{fig:}}
% \subfigure[]{\includegraphics[width=0.45\linewidth]{./figures/empty.eps}\label{fig:}}
% \caption{\pavlos{Comparison of different measurement selection policies. Average number of nodes with certain color after measurement (y-axis) for different measurement budgets (x-axis).} \pavlos{NOTE: we have not yet designed the policies.} }
% \label{fig:}
% \end{figure}

% \begin{figure}
% \centering
% \subfigure[]{\includegraphics[width=0.45\linewidth]{./figures/empty.eps}\label{fig:}}
% \subfigure[]{\includegraphics[width=0.45\linewidth]{./figures/empty.eps}\label{fig:}}
% \caption{\pavlos{Statistics of the network properties (\eg centrality, degree, ISP/stub, etc.) of the nodes selected as good vantage points by the XXX and YYY measurement policies.}}
% \label{fig:}
% \end{figure}


==> RouteEntropy.tex <==
\myitem{Route Entropy: A measure of route uncertainty.}
\vkotronis{Candidate for removal!}
\blue{
In this section, we introduce the metric of \textit{route entropy} to quantify the uncertainty in a network and routing configuration. Similarly to the information-theoretic definition of entropy, the more uncertainty we have for the catchment, the higher the value of the route entropy.
\begin{definition}[Route Entropy]
The \emph{route entropy of a node $i$} is defined as:
\begin{equation}
H(i) = -\sum_{m\in\mathcal{M}}\pi_{i}(m)\cdot \log\left(\pi_{i}(m)\right)
\end{equation}
where $\mathcal{M}$, the set of \ppoints. The \emph{mutual route entropy of a set of nodes} $S\subseteq \mathcal{N}_{R}$ is defined as
\begin{equation}
    H(S) = -\sum_{x\in \mathcal{M}^{|S|}} P(S\rhd x)\cdot \log\left(P(S\rhd x)\right)
\end{equation}
where $x$ is a vector of length $|S|$ ($x\in \mathcal{M}^{|S|}$), and $P(S\rhd x) = Prob\{\bigcup_{i\in S}~ \bestaspath{i}{n_{dst}}\rhd x_{i}\}$.
\end{definition}
}
%\vkotronis{\emph{Note that $\mathcal{M}^{|S|}$ is expressing all possible combinations of $\mathcal{M}$ in a vector of length $|S|$.}}

\blue{
The route entropy of a node, denotes how ``evenly spread'' its route probabilities are. For example, for $M=2$, a node $i$ that has equal probabilities to route through any of the two \ppoints, i.e., $\pi_{i}(1) = \pi_{i}(2)=0.5$, has higher entropy than a node $j$ that is more probable to route through one of the \ppoints, e.g., $\pi_{j}(1)=0.8$ and $\pi_{j}(2)=0.2$. The route entropy for a node with certain route is zero.
} 
%\pavlos{In other words, the route entropy tells you how much information you learn, on average, when someone tells you that a node routes through a \ppoint.}
\blue{
Similarly, the entropy of the entire \Rgraph, $H(\mathcal{N_{R}})$, can be used as a measure of uncertainty of a routing configuration. However, to calculate the exact value of $H(\mathcal{N_{R}})$ is a complex task, since it requires to calculate the joint distribution of $P(\mathcal{N_{R}} \rhd x)$, $x\in\mathcal{M}^{|\mathcal{N}_{R}|}$, whose state space is exponential to the number of nodes. An upper bound for the mutual entropy is given by the sum of the route entropies of the individual nodes, i.e., $H(S) \leq \sum_{i\in S} H(i)$; the calculation of this bound requires $\Theta\left(|\mathcal{M}|\cdot|\mathcal{N}_{R}|\right)$ calculations, which is linear to the number of nodes.
}

\pavlos{An application of the above quantity is to know what is the importance by learning a routing policy (for which we have uncertainty) or measuring a node.}

%\vkotronis{Great idea! We may also use the hegemony index to see if there is any correlation, e.g., if measuring a node with a high heg. index bring significant decrease in entropy, and similarly with low heg. index. This can go into the measurement-assisted inference I suppose. What do you think?}
